Compact Example-Based Explanations for Language Models

Training data influence estimation methods quantify the contribution of training documents to a model's output, making them a promising source of information for example-based explanations. As humans cannot interpret thousands of documents, only a small subset of the training data can be presented as an explanation. Although the choice of which documents to include directly affects explanation quality, previous evaluations of such systems have largely ignored any selection strategies. To address this, we propose a novel selection relevance score, a retraining-free metric that quantifies how useful a set of examples is for explaining a model's output. We validate this score through fine-tuning experiments, confirming that it can predict whether a set of examples supports or undermines the model's predictions. Using this metric, we further show that common selection strategies often underperform random selection. Motivated by this finding, we propose a strategy that balances influence and representativeness, enabling better use of selection budgets than naively selecting the highest-ranking examples.

==> tables/scoring/pred_gain/full_per_estimator_model_selection.tex <==
\begin{tabular}{l|l|l}
\toprule
\midrule
Olmo2-1B & most inf. & {\cellcolor[HTML]{FFF7FB}} \color[HTML]{000000} -28.76 dB \\
Olmo2-1B & most inf. & {\cellcolor[HTML]{FBF3F9}} \color[HTML]{000000} -26.65 dB \\
Olmo2-1B & most harmful & {\cellcolor[HTML]{FAF2F8}} \color[HTML]{000000} -25.95 dB \\
Olmo2-1B & most harmful & {\cellcolor[HTML]{F9F2F8}} \color[HTML]{000000} -25.54 dB \\
Olmo2-1B & most helpful & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -25.28 dB \\
Qwen2.5-0.5B & most inf. & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -25.07 dB \\
Qwen2.5-0.5B & most inf. & {\cellcolor[HTML]{F7F0F7}} \color[HTML]{000000} -24.44 dB \\
Olmo2-1B & most helpful & {\cellcolor[HTML]{F7F0F7}} \color[HTML]{000000} -24.43 dB \\
Qwen2.5-0.5B & most harmful & {\cellcolor[HTML]{F6EFF7}} \color[HTML]{000000} -24.03 dB \\
Olmo2-1B &  AIDE & {\cellcolor[HTML]{F5EFF6}} \color[HTML]{000000} -23.89 dB \\
Qwen2.5-0.5B & most helpful & {\cellcolor[HTML]{F5EFF6}} \color[HTML]{000000} -23.85 dB \\
Qwen2.5-0.5B & most helpful & {\cellcolor[HTML]{F5EFF6}} \color[HTML]{000000} -23.77 dB \\
Qwen2.5-0.5B & most harmful & {\cellcolor[HTML]{F4EEF6}} \color[HTML]{000000} -23.30 dB \\
Olmo2-1B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{F4EDF6}} \color[HTML]{000000} -23.02 dB \\
Olmo2-1B &  DIVINE most inf. & {\cellcolor[HTML]{F4EDF6}} \color[HTML]{000000} -23.01 dB \\
Olmo2-1B &  AIDE & {\cellcolor[HTML]{F4EDF6}} \color[HTML]{000000} -22.94 dB \\
Olmo2-1B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{F3EDF5}} \color[HTML]{000000} -22.70 dB \\
Olmo2-1B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{F2ECF5}} \color[HTML]{000000} -22.44 dB \\
Olmo2-1B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{F2ECF5}} \color[HTML]{000000} -22.28 dB \\
Olmo2-1B &  DIVINE most harmful & {\cellcolor[HTML]{F2ECF5}} \color[HTML]{000000} -22.14 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{F2ECF5}} \color[HTML]{000000} -22.10 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{F2ECF5}} \color[HTML]{000000} -22.09 dB \\
Olmo2-1B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{F2ECF5}} \color[HTML]{000000} -22.08 dB \\
Qwen2.5-0.5B &  DIVINE most inf. & {\cellcolor[HTML]{F2ECF5}} \color[HTML]{000000} -22.03 dB \\
Olmo2-1B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{F2ECF5}} \color[HTML]{000000} -22.00 dB \\
Olmo2-1B &  FL most harmful $\lambda=.25$ & {\cellcolor[HTML]{F2ECF5}} \color[HTML]{000000} -21.99 dB \\
Qwen2.5-0.5B &  DIVINE most inf. & {\cellcolor[HTML]{F1EBF5}} \color[HTML]{000000} -21.82 dB \\
Olmo2-1B &  FL most harmful $\lambda=.25$ & {\cellcolor[HTML]{F1EBF5}} \color[HTML]{000000} -21.81 dB \\
Olmo2-1B &  FL most helpful $\lambda=.25$ & {\cellcolor[HTML]{F1EBF5}} \color[HTML]{000000} -21.75 dB \\
Qwen2.5-0.5B &  AIDE & {\cellcolor[HTML]{F1EBF5}} \color[HTML]{000000} -21.71 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{F1EBF5}} \color[HTML]{000000} -21.70 dB \\
Qwen2.5-0.5B &  FL most helpful $\lambda=.25$ & {\cellcolor[HTML]{F1EBF5}} \color[HTML]{000000} -21.69 dB \\
Olmo2-1B &  FL most harmful $\lambda=.5$ & {\cellcolor[HTML]{F1EBF5}} \color[HTML]{000000} -21.68 dB \\
Olmo2-1B &  FL most harmful $\lambda=.5$ & {\cellcolor[HTML]{F1EBF5}} \color[HTML]{000000} -21.62 dB \\
Qwen2.5-0.5B &  AIDE & {\cellcolor[HTML]{F1EBF4}} \color[HTML]{000000} -21.58 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{F1EBF4}} \color[HTML]{000000} -21.57 dB \\
Olmo2-1B &  DIVINE most helpful & {\cellcolor[HTML]{F1EBF4}} \color[HTML]{000000} -21.55 dB \\
Olmo2-1B &  FL most helpful $\lambda=.5$ & {\cellcolor[HTML]{F1EBF4}} \color[HTML]{000000} -21.53 dB \\
Qwen2.5-0.5B &  FL most harmful $\lambda=.25$ & {\cellcolor[HTML]{F1EBF4}} \color[HTML]{000000} -21.46 dB \\
Qwen2.5-0.5B &  FL most helpful $\lambda=.5$ & {\cellcolor[HTML]{F1EBF4}} \color[HTML]{000000} -21.40 dB \\
Olmo2-1B &  FL most harmful $\lambda=.75$ & {\cellcolor[HTML]{F1EBF4}} \color[HTML]{000000} -21.39 dB \\
Qwen2.5-0.5B &  FL most harmful $\lambda=.25$ & {\cellcolor[HTML]{F1EBF4}} \color[HTML]{000000} -21.38 dB \\
Olmo2-1B &  FL most helpful $\lambda=.25$ & {\cellcolor[HTML]{F1EBF4}} \color[HTML]{000000} -21.38 dB \\
Olmo2-1B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{F1EBF4}} \color[HTML]{000000} -21.35 dB \\
Qwen2.5-0.5B &  FL most helpful $\lambda=.25$ & {\cellcolor[HTML]{F1EBF4}} \color[HTML]{000000} -21.34 dB \\
Qwen2.5-0.5B &  DIVINE most helpful & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -21.26 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -21.22 dB \\
Olmo2-1B &  FL most helpful $\lambda=.5$ & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -21.19 dB \\
Qwen2.5-0.5B &  FL most helpful $\lambda=.5$ & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -21.13 dB \\
Olmo2-1B &  FL most helpful $\lambda=.75$ & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -21.13 dB \\
Olmo2-1B &  DIVINE most helpful & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -21.10 dB \\
Qwen2.5-0.5B &  DIVINE most harmful & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -21.08 dB \\
Qwen2.5-0.5B &  DIVINE most helpful & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -20.92 dB \\
Qwen2.5-0.5B &  DIVINE most harmful & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -20.90 dB \\
Qwen2.5-0.5B &  FL most harmful $\lambda=.5$ & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -20.87 dB \\
Qwen2.5-0.5B &  FL most helpful $\lambda=.75$ & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -20.86 dB \\
Olmo2-1B &  FL most helpful $\lambda=.75$ & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -20.76 dB \\
Qwen2.5-0.5B &  FL most helpful $\lambda=.75$ & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -20.72 dB \\
Olmo2-1B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{EFE9F3}} \color[HTML]{000000} -20.69 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{EFE9F3}} \color[HTML]{000000} -20.60 dB \\
Llama-3.2-1B & most harmful & {\cellcolor[HTML]{EFE9F3}} \color[HTML]{000000} -20.54 dB \\
Qwen2.5-0.5B &  FL most harmful $\lambda=.75$ & {\cellcolor[HTML]{EFE9F3}} \color[HTML]{000000} -20.52 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{EFE9F3}} \color[HTML]{000000} -20.47 dB \\
Qwen2.5-0.5B &  FL most harmful $\lambda=.5$ & {\cellcolor[HTML]{EFE9F3}} \color[HTML]{000000} -20.44 dB \\
Llama-3.2-1B & most inf. & {\cellcolor[HTML]{EEE9F3}} \color[HTML]{000000} -20.37 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{EEE9F3}} \color[HTML]{000000} -20.29 dB \\
Llama-3.2-1B & most inf. & {\cellcolor[HTML]{EEE8F3}} \color[HTML]{000000} -20.08 dB \\
Llama-3.2-1B & most harmful & {\cellcolor[HTML]{EEE8F3}} \color[HTML]{000000} -20.04 dB \\
Olmo2-1B &  FL most harmful $\lambda=1$ & {\cellcolor[HTML]{EEE8F3}} \color[HTML]{000000} -20.02 dB \\
Qwen2.5-0.5B &  FL most harmful $\lambda=.75$ & {\cellcolor[HTML]{EEE8F3}} \color[HTML]{000000} -20.01 dB \\
Llama-3.2-1B & most helpful & {\cellcolor[HTML]{EEE8F3}} \color[HTML]{000000} -19.85 dB \\
Qwen2.5-0.5B &  FL most helpful $\lambda=1$ & {\cellcolor[HTML]{EEE8F3}} \color[HTML]{000000} -19.82 dB \\
Qwen2.5-0.5B &  FL most harmful $\lambda=1$ & {\cellcolor[HTML]{EDE8F3}} \color[HTML]{000000} -19.71 dB \\
Qwen2.5-0.5B &  FL most helpful $\lambda=1$ & {\cellcolor[HTML]{EDE8F3}} \color[HTML]{000000} -19.65 dB \\
Qwen2.5-0.5B &  FL most harmful $\lambda=1$ & {\cellcolor[HTML]{EDE8F3}} \color[HTML]{000000} -19.54 dB \\
Olmo2-1B &  FL most helpful $\lambda=1$ & {\cellcolor[HTML]{EDE7F2}} \color[HTML]{000000} -19.49 dB \\
Llama-3.2-1B &  FL most harmful $\lambda=.25$ & {\cellcolor[HTML]{EDE7F2}} \color[HTML]{000000} -19.46 dB \\
Olmo2-1B &  FL most helpful $\lambda=1$ & {\cellcolor[HTML]{EDE7F2}} \color[HTML]{000000} -19.34 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{EDE7F2}} \color[HTML]{000000} -19.34 dB \\
Llama-3.2-1B & most helpful & {\cellcolor[HTML]{EDE7F2}} \color[HTML]{000000} -19.26 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{EDE7F2}} \color[HTML]{000000} -19.26 dB \\
Llama-3.2-1B &  AIDE & {\cellcolor[HTML]{EDE7F2}} \color[HTML]{000000} -19.24 dB \\
Llama-3.2-1B &  FL most harmful $\lambda=.25$ & {\cellcolor[HTML]{EDE7F2}} \color[HTML]{000000} -19.22 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{ECE7F2}} \color[HTML]{000000} -19.13 dB \\
Llama-3.2-1B &  FL most harmful $\lambda=.5$ & {\cellcolor[HTML]{ECE7F2}} \color[HTML]{000000} -19.13 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{ECE7F2}} \color[HTML]{000000} -19.00 dB \\
Olmo2-1B &  FL most harmful $\lambda=.75$ & {\cellcolor[HTML]{ECE7F2}} \color[HTML]{000000} -18.95 dB \\
Llama-3.2-1B &  FL most helpful $\lambda=.25$ & {\cellcolor[HTML]{ECE7F2}} \color[HTML]{000000} -18.95 dB \\
Llama-3.2-1B &  FL most harmful $\lambda=.5$ & {\cellcolor[HTML]{ECE7F2}} \color[HTML]{000000} -18.92 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{EBE6F2}} \color[HTML]{000000} -18.89 dB \\
Llama-3.2-1B &  FL most harmful $\lambda=.75$ & {\cellcolor[HTML]{EBE6F2}} \color[HTML]{000000} -18.89 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{EBE6F2}} \color[HTML]{000000} -18.85 dB \\
Llama-3.2-1B &  FL most harmful $\lambda=.75$ & {\cellcolor[HTML]{EBE6F2}} \color[HTML]{000000} -18.79 dB \\
Llama-3.2-1B &  AIDE & {\cellcolor[HTML]{EBE6F2}} \color[HTML]{000000} -18.76 dB \\
Llama-3.2-1B &  FL most helpful $\lambda=.5$ & {\cellcolor[HTML]{EBE6F2}} \color[HTML]{000000} -18.63 dB \\
Llama-3.2-1B &  FL most helpful $\lambda=.25$ & {\cellcolor[HTML]{EAE6F1}} \color[HTML]{000000} -18.31 dB \\
Llama-3.2-1B &  DIVINE most harmful & {\cellcolor[HTML]{E9E5F1}} \color[HTML]{000000} -18.29 dB \\
Llama-3.2-1B &  DIVINE most harmful & {\cellcolor[HTML]{E9E5F1}} \color[HTML]{000000} -18.28 dB \\
Llama-3.2-1B &  DIVINE most inf. & {\cellcolor[HTML]{E9E5F1}} \color[HTML]{000000} -18.11 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{E9E5F1}} \color[HTML]{000000} -18.10 dB \\
Llama-3.2-1B &  FL most harmful $\lambda=1$ & {\cellcolor[HTML]{E9E5F1}} \color[HTML]{000000} -18.10 dB \\
Llama-3.2-1B &  FL most helpful $\lambda=.5$ & {\cellcolor[HTML]{E9E5F1}} \color[HTML]{000000} -18.08 dB \\
Olmo2-1B &  FL most harmful $\lambda=1$ & {\cellcolor[HTML]{E9E5F1}} \color[HTML]{000000} -18.07 dB \\
Llama-3.2-1B &  FL most harmful $\lambda=1$ & {\cellcolor[HTML]{E9E5F1}} \color[HTML]{000000} -18.05 dB \\
Llama-3.2-1B &  DIVINE most inf. & {\cellcolor[HTML]{E9E5F1}} \color[HTML]{000000} -18.03 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{E8E4F0}} \color[HTML]{000000} -18.00 dB \\
Llama-3.2-1B &  FL most helpful $\lambda=.75$ & {\cellcolor[HTML]{E8E4F0}} \color[HTML]{000000} -17.98 dB \\
Olmo2-1B &  DIVINE most inf. & {\cellcolor[HTML]{E8E4F0}} \color[HTML]{000000} -17.98 dB \\
Llama-3.2-1B &  DIVINE most helpful & {\cellcolor[HTML]{E7E3F0}} \color[HTML]{000000} -17.61 dB \\
Llama-3.2-1B &  FL most helpful $\lambda=.75$ & {\cellcolor[HTML]{E7E3F0}} \color[HTML]{000000} -17.60 dB \\
Llama-3.2-1B &  DIVINE most helpful & {\cellcolor[HTML]{E6E2EF}} \color[HTML]{000000} -16.88 dB \\
Llama-3.2-1B &  FL most helpful $\lambda=1$ & {\cellcolor[HTML]{E5E1EF}} \color[HTML]{000000} -16.55 dB \\
Llama-3.2-1B &  FL most helpful $\lambda=1$ & {\cellcolor[HTML]{E4E1EF}} \color[HTML]{000000} -16.37 dB \\
Olmo2-1B &  DIVINE most harmful & {\cellcolor[HTML]{E3E0EE}} \color[HTML]{000000} -16.22 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{B5C4DF}} \color[HTML]{000000} -3.60 dB \\
Qwen2.5-0.5B & random & {\cellcolor[HTML]{B4C4DF}} \color[HTML]{000000} -3.23 dB \\
Olmo2-1B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{B3C3DE}} \color[HTML]{000000} -3.07 dB \\
Llama-3.2-1B & random & {\cellcolor[HTML]{B3C3DE}} \color[HTML]{000000} -2.92 dB \\
Olmo2-1B & random & {\cellcolor[HTML]{B3C3DE}} \color[HTML]{000000} -2.81 dB \\
Qwen2.5-0.5B &  DIVINE least inf. & {\cellcolor[HTML]{B0C2DE}} \color[HTML]{000000} -2.36 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{AFC1DD}} \color[HTML]{000000} -2.00 dB \\
Olmo2-1B &  DIVINE least inf. & {\cellcolor[HTML]{ADC1DD}} \color[HTML]{000000} -1.74 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{ADC1DD}} \color[HTML]{000000} -1.59 dB \\
Llama-3.2-1B &  DIVINE least inf. & {\cellcolor[HTML]{ACC0DD}} \color[HTML]{000000} -1.52 dB \\
Olmo2-1B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{ACC0DD}} \color[HTML]{000000} -1.41 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{ACC0DD}} \color[HTML]{000000} -1.30 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{ABBFDC}} \color[HTML]{000000} -1.20 dB \\
Qwen2.5-0.5B & least inf. & {\cellcolor[HTML]{ABBFDC}} \color[HTML]{000000} -1.19 dB \\
Olmo2-1B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{ABBFDC}} \color[HTML]{000000} -1.17 dB \\
Olmo2-1B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{ABBFDC}} \color[HTML]{000000} -1.04 dB \\
Olmo2-1B & least inf. & {\cellcolor[HTML]{A9BFDC}} \color[HTML]{000000} -0.97 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{A9BFDC}} \color[HTML]{000000} -0.85 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{A8BEDC}} \color[HTML]{000000} -0.67 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{A8BEDC}} \color[HTML]{000000} -0.54 dB \\
Llama-3.2-1B & least inf. & {\cellcolor[HTML]{A8BEDC}} \color[HTML]{000000} -0.48 dB \\
Olmo2-1B & least inf. & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.19 dB \\
Olmo2-1B &  DIVINE least inf. & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.19 dB \\
Olmo2-1B & least inf. & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.19 dB \\
Olmo2-1B &  DIVINE least inf. & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.19 dB \\
Olmo2-1B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.18 dB \\
Olmo2-1B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.18 dB \\
Olmo2-1B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.18 dB \\
Olmo2-1B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.18 dB \\
Olmo2-1B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.18 dB \\
Olmo2-1B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.18 dB \\
Olmo2-1B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.18 dB \\
Olmo2-1B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.18 dB \\
Qwen2.5-0.5B &  DIVINE least inf. & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.14 dB \\
Qwen2.5-0.5B & least inf. & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.14 dB \\
Qwen2.5-0.5B &  DIVINE least inf. & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.14 dB \\
Qwen2.5-0.5B & least inf. & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.14 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.13 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.13 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.13 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.13 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.13 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.13 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.13 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.13 dB \\
Llama-3.2-1B &  DIVINE least inf. & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.10 dB \\
Llama-3.2-1B & least inf. & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.10 dB \\
Llama-3.2-1B &  DIVINE least inf. & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.10 dB \\
Llama-3.2-1B & least inf. & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.10 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.09 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.09 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.09 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{A7BDDB}} \color[HTML]{000000} -0.09 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{A5BDDB}} \color[HTML]{000000} -0.09 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{A5BDDB}} \color[HTML]{000000} -0.09 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{A5BDDB}} \color[HTML]{000000} -0.09 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{A5BDDB}} \color[HTML]{000000} -0.09 dB \\
Olmo2-1B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{569DC8}} \color[HTML]{F1F1F1} 14.08 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{4E9AC6}} \color[HTML]{F1F1F1} 15.24 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{4094C3}} \color[HTML]{F1F1F1} 17.24 dB \\
Olmo2-1B &  DIVINE most inf. & {\cellcolor[HTML]{308CBE}} \color[HTML]{F1F1F1} 19.92 dB \\
Olmo2-1B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{2D8ABD}} \color[HTML]{F1F1F1} 20.65 dB \\
Olmo2-1B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{2D8ABD}} \color[HTML]{F1F1F1} 20.78 dB \\
Olmo2-1B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{2C89BD}} \color[HTML]{F1F1F1} 20.90 dB \\
Olmo2-1B & most inf. & {\cellcolor[HTML]{2C89BD}} \color[HTML]{F1F1F1} 20.98 dB \\
Olmo2-1B &  AIDE & {\cellcolor[HTML]{2987BC}} \color[HTML]{F1F1F1} 21.59 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{0F76B3}} \color[HTML]{F1F1F1} 26.65 dB \\
Llama-3.2-1B &  AIDE & {\cellcolor[HTML]{0F76B3}} \color[HTML]{F1F1F1} 26.69 dB \\
Llama-3.2-1B & most inf. & {\cellcolor[HTML]{0F76B3}} \color[HTML]{F1F1F1} 26.71 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{0F76B3}} \color[HTML]{F1F1F1} 26.71 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{0D75B3}} \color[HTML]{F1F1F1} 27.01 dB \\
Llama-3.2-1B &  DIVINE most inf. & {\cellcolor[HTML]{0771B1}} \color[HTML]{F1F1F1} 28.21 dB \\
Qwen2.5-0.5B & most inf. & {\cellcolor[HTML]{056DAB}} \color[HTML]{F1F1F1} 29.82 dB \\
Qwen2.5-0.5B &  AIDE & {\cellcolor[HTML]{056DAB}} \color[HTML]{F1F1F1} 29.87 dB \\
Qwen2.5-0.5B &  DIVINE most inf. & {\cellcolor[HTML]{0569A5}} \color[HTML]{F1F1F1} 31.33 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{05659F}} \color[HTML]{F1F1F1} 33.21 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{04649E}} \color[HTML]{F1F1F1} 33.42 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{04649E}} \color[HTML]{F1F1F1} 33.45 dB \\
Olmo2-1B & Test instance & {\cellcolor[HTML]{045585}} \color[HTML]{F1F1F1} 39.40 dB \\
Olmo2-1B & Test instance & {\cellcolor[HTML]{045585}} \color[HTML]{F1F1F1} 39.40 dB \\
Olmo2-1B & Test instance & {\cellcolor[HTML]{045585}} \color[HTML]{F1F1F1} 39.40 dB \\
Llama-3.2-1B & Test instance & {\cellcolor[HTML]{03456C}} \color[HTML]{F1F1F1} 44.03 dB \\
Llama-3.2-1B & Test instance & {\cellcolor[HTML]{03456C}} \color[HTML]{F1F1F1} 44.03 dB \\
Llama-3.2-1B & Test instance & {\cellcolor[HTML]{03456C}} \color[HTML]{F1F1F1} 44.03 dB \\
Qwen2.5-0.5B & Test instance & {\cellcolor[HTML]{023858}} \color[HTML]{F1F1F1} 47.70 dB \\
Qwen2.5-0.5B & Test instance & {\cellcolor[HTML]{023858}} \color[HTML]{F1F1F1} 47.70 dB \\
Qwen2.5-0.5B & Test instance & {\cellcolor[HTML]{023858}} \color[HTML]{F1F1F1} 47.70 dB \\
\bottomrule
\end{tabular}


==> tables/scoring/pred_gain/full_per_estimator_model_selection_k_10.tex <==
\begin{tabular}{l|l|l}
\toprule
\midrule
Olmo2-1B & most inf. & {\cellcolor[HTML]{FFF7FB}} \color[HTML]{000000} -28.72 dB \\
Olmo2-1B & most inf. & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -25.95 dB \\
Olmo2-1B & most harmful & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -25.82 dB \\
Olmo2-1B & most harmful & {\cellcolor[HTML]{F6EFF7}} \color[HTML]{000000} -24.99 dB \\
Olmo2-1B & most helpful & {\cellcolor[HTML]{F5EFF6}} \color[HTML]{000000} -24.76 dB \\
Qwen2.5-0.5B & most inf. & {\cellcolor[HTML]{F5EEF6}} \color[HTML]{000000} -24.48 dB \\
Olmo2-1B & most helpful & {\cellcolor[HTML]{F4EEF6}} \color[HTML]{000000} -24.08 dB \\
Qwen2.5-0.5B & most inf. & {\cellcolor[HTML]{F4EDF6}} \color[HTML]{000000} -23.91 dB \\
Olmo2-1B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{F3EDF5}} \color[HTML]{000000} -23.64 dB \\
Qwen2.5-0.5B & most harmful & {\cellcolor[HTML]{F3EDF5}} \color[HTML]{000000} -23.62 dB \\
Qwen2.5-0.5B & most helpful & {\cellcolor[HTML]{F2ECF5}} \color[HTML]{000000} -23.56 dB \\
Qwen2.5-0.5B & most helpful & {\cellcolor[HTML]{F2ECF5}} \color[HTML]{000000} -23.53 dB \\
Olmo2-1B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{F2ECF5}} \color[HTML]{000000} -23.21 dB \\
Olmo2-1B &  AIDE & {\cellcolor[HTML]{F2ECF5}} \color[HTML]{000000} -23.12 dB \\
Olmo2-1B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{F1EBF5}} \color[HTML]{000000} -22.84 dB \\
Qwen2.5-0.5B & most harmful & {\cellcolor[HTML]{F1EBF5}} \color[HTML]{000000} -22.82 dB \\
Olmo2-1B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{F1EBF4}} \color[HTML]{000000} -22.70 dB \\
Olmo2-1B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{F1EBF4}} \color[HTML]{000000} -22.61 dB \\
Olmo2-1B &  FL most harmful $\lambda=.25$ & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -22.41 dB \\
Olmo2-1B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -22.39 dB \\
Olmo2-1B &  AIDE & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -22.37 dB \\
Olmo2-1B &  DIVINE most inf. & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -22.24 dB \\
Olmo2-1B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -22.22 dB \\
Olmo2-1B &  FL most harmful $\lambda=.25$ & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -22.08 dB \\
Olmo2-1B &  FL most harmful $\lambda=.5$ & {\cellcolor[HTML]{EFE9F3}} \color[HTML]{000000} -22.06 dB \\
Olmo2-1B &  FL most helpful $\lambda=.25$ & {\cellcolor[HTML]{EFE9F3}} \color[HTML]{000000} -22.01 dB \\
Olmo2-1B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{EFE9F3}} \color[HTML]{000000} -21.91 dB \\
Olmo2-1B &  FL most harmful $\lambda=.5$ & {\cellcolor[HTML]{EFE9F3}} \color[HTML]{000000} -21.85 dB \\
Olmo2-1B &  FL most helpful $\lambda=.5$ & {\cellcolor[HTML]{EEE9F3}} \color[HTML]{000000} -21.81 dB \\
Olmo2-1B &  DIVINE most harmful & {\cellcolor[HTML]{EEE9F3}} \color[HTML]{000000} -21.65 dB \\
Olmo2-1B &  FL most harmful $\lambda=.75$ & {\cellcolor[HTML]{EEE9F3}} \color[HTML]{000000} -21.62 dB \\
Olmo2-1B &  FL most helpful $\lambda=.25$ & {\cellcolor[HTML]{EEE9F3}} \color[HTML]{000000} -21.62 dB \\
Olmo2-1B &  FL most harmful $\lambda=.75$ & {\cellcolor[HTML]{EEE8F3}} \color[HTML]{000000} -21.56 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{EEE8F3}} \color[HTML]{000000} -21.54 dB \\
Olmo2-1B &  FL most helpful $\lambda=.75$ & {\cellcolor[HTML]{EEE8F3}} \color[HTML]{000000} -21.43 dB \\
Olmo2-1B &  FL most helpful $\lambda=.5$ & {\cellcolor[HTML]{EDE8F3}} \color[HTML]{000000} -21.29 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{EDE8F3}} \color[HTML]{000000} -21.29 dB \\
Qwen2.5-0.5B &  AIDE & {\cellcolor[HTML]{EDE8F3}} \color[HTML]{000000} -21.21 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{EDE8F3}} \color[HTML]{000000} -21.19 dB \\
Qwen2.5-0.5B &  FL most helpful $\lambda=.25$ & {\cellcolor[HTML]{EDE8F3}} \color[HTML]{000000} -21.18 dB \\
Olmo2-1B &  DIVINE most helpful & {\cellcolor[HTML]{EDE8F3}} \color[HTML]{000000} -21.14 dB \\
Qwen2.5-0.5B &  DIVINE most inf. & {\cellcolor[HTML]{EDE8F3}} \color[HTML]{000000} -21.11 dB \\
Qwen2.5-0.5B &  DIVINE most inf. & {\cellcolor[HTML]{EDE7F2}} \color[HTML]{000000} -21.00 dB \\
Qwen2.5-0.5B &  DIVINE most helpful & {\cellcolor[HTML]{EDE7F2}} \color[HTML]{000000} -20.87 dB \\
Qwen2.5-0.5B &  FL most helpful $\lambda=.5$ & {\cellcolor[HTML]{EDE7F2}} \color[HTML]{000000} -20.85 dB \\
Olmo2-1B &  FL most helpful $\lambda=.75$ & {\cellcolor[HTML]{ECE7F2}} \color[HTML]{000000} -20.83 dB \\
Qwen2.5-0.5B &  FL most harmful $\lambda=.25$ & {\cellcolor[HTML]{ECE7F2}} \color[HTML]{000000} -20.83 dB \\
Qwen2.5-0.5B &  AIDE & {\cellcolor[HTML]{ECE7F2}} \color[HTML]{000000} -20.73 dB \\
Qwen2.5-0.5B &  FL most helpful $\lambda=.25$ & {\cellcolor[HTML]{ECE7F2}} \color[HTML]{000000} -20.62 dB \\
Olmo2-1B &  FL most harmful $\lambda=1$ & {\cellcolor[HTML]{ECE7F2}} \color[HTML]{000000} -20.60 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{EBE6F2}} \color[HTML]{000000} -20.55 dB \\
Qwen2.5-0.5B &  FL most harmful $\lambda=.25$ & {\cellcolor[HTML]{EBE6F2}} \color[HTML]{000000} -20.54 dB \\
Qwen2.5-0.5B &  FL most helpful $\lambda=.5$ & {\cellcolor[HTML]{EBE6F2}} \color[HTML]{000000} -20.44 dB \\
Olmo2-1B &  DIVINE most helpful & {\cellcolor[HTML]{EBE6F2}} \color[HTML]{000000} -20.39 dB \\
Qwen2.5-0.5B &  DIVINE most harmful & {\cellcolor[HTML]{EBE6F2}} \color[HTML]{000000} -20.38 dB \\
Olmo2-1B &  FL most harmful $\lambda=1$ & {\cellcolor[HTML]{EAE6F1}} \color[HTML]{000000} -20.32 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{EAE6F1}} \color[HTML]{000000} -20.20 dB \\
Qwen2.5-0.5B &  FL most helpful $\lambda=.75$ & {\cellcolor[HTML]{EAE6F1}} \color[HTML]{000000} -20.20 dB \\
Qwen2.5-0.5B &  DIVINE most helpful & {\cellcolor[HTML]{EAE6F1}} \color[HTML]{000000} -20.18 dB \\
Qwen2.5-0.5B &  DIVINE most harmful & {\cellcolor[HTML]{EAE6F1}} \color[HTML]{000000} -20.11 dB \\
Qwen2.5-0.5B &  FL most harmful $\lambda=.5$ & {\cellcolor[HTML]{E9E5F1}} \color[HTML]{000000} -20.06 dB \\
Olmo2-1B &  FL most helpful $\lambda=1$ & {\cellcolor[HTML]{E9E5F1}} \color[HTML]{000000} -20.05 dB \\
Llama-3.2-1B & most harmful & {\cellcolor[HTML]{E9E5F1}} \color[HTML]{000000} -20.04 dB \\
Qwen2.5-0.5B &  FL most helpful $\lambda=.75$ & {\cellcolor[HTML]{E9E5F1}} \color[HTML]{000000} -19.97 dB \\
Olmo2-1B &  FL most helpful $\lambda=1$ & {\cellcolor[HTML]{E8E4F0}} \color[HTML]{000000} -19.82 dB \\
Qwen2.5-0.5B &  FL most harmful $\lambda=.75$ & {\cellcolor[HTML]{E8E4F0}} \color[HTML]{000000} -19.80 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{E8E4F0}} \color[HTML]{000000} -19.77 dB \\
Llama-3.2-1B & most inf. & {\cellcolor[HTML]{E8E4F0}} \color[HTML]{000000} -19.76 dB \\
Qwen2.5-0.5B &  FL most helpful $\lambda=1$ & {\cellcolor[HTML]{E7E3F0}} \color[HTML]{000000} -19.61 dB \\
Llama-3.2-1B & most inf. & {\cellcolor[HTML]{E7E3F0}} \color[HTML]{000000} -19.53 dB \\
Llama-3.2-1B & most helpful & {\cellcolor[HTML]{E7E3F0}} \color[HTML]{000000} -19.42 dB \\
Llama-3.2-1B & most harmful & {\cellcolor[HTML]{E7E3F0}} \color[HTML]{000000} -19.41 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{E7E3F0}} \color[HTML]{000000} -19.34 dB \\
Qwen2.5-0.5B &  FL most harmful $\lambda=1$ & {\cellcolor[HTML]{E7E3F0}} \color[HTML]{000000} -19.29 dB \\
Qwen2.5-0.5B &  FL most helpful $\lambda=1$ & {\cellcolor[HTML]{E7E3F0}} \color[HTML]{000000} -19.27 dB \\
Qwen2.5-0.5B &  FL most harmful $\lambda=1$ & {\cellcolor[HTML]{E7E3F0}} \color[HTML]{000000} -19.19 dB \\
Llama-3.2-1B &  AIDE & {\cellcolor[HTML]{E7E3F0}} \color[HTML]{000000} -19.14 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{E6E2EF}} \color[HTML]{000000} -19.05 dB \\
Qwen2.5-0.5B &  FL most harmful $\lambda=.5$ & {\cellcolor[HTML]{E6E2EF}} \color[HTML]{000000} -19.02 dB \\
Qwen2.5-0.5B &  FL most harmful $\lambda=.75$ & {\cellcolor[HTML]{E6E2EF}} \color[HTML]{000000} -18.90 dB \\
Llama-3.2-1B &  FL most harmful $\lambda=.25$ & {\cellcolor[HTML]{E5E1EF}} \color[HTML]{000000} -18.81 dB \\
Llama-3.2-1B & most helpful & {\cellcolor[HTML]{E5E1EF}} \color[HTML]{000000} -18.73 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{E4E1EF}} \color[HTML]{000000} -18.58 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{E4E1EF}} \color[HTML]{000000} -18.55 dB \\
Llama-3.2-1B &  AIDE & {\cellcolor[HTML]{E4E1EF}} \color[HTML]{000000} -18.53 dB \\
Llama-3.2-1B &  FL most harmful $\lambda=.5$ & {\cellcolor[HTML]{E4E1EF}} \color[HTML]{000000} -18.45 dB \\
Llama-3.2-1B &  FL most harmful $\lambda=.25$ & {\cellcolor[HTML]{E4E1EF}} \color[HTML]{000000} -18.40 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{E3E0EE}} \color[HTML]{000000} -18.34 dB \\
Llama-3.2-1B &  FL most helpful $\lambda=.25$ & {\cellcolor[HTML]{E3E0EE}} \color[HTML]{000000} -18.29 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{E3E0EE}} \color[HTML]{000000} -18.18 dB \\
Llama-3.2-1B &  FL most harmful $\lambda=.75$ & {\cellcolor[HTML]{E3E0EE}} \color[HTML]{000000} -18.14 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{E2DFEE}} \color[HTML]{000000} -18.14 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{E2DFEE}} \color[HTML]{000000} -18.05 dB \\
Llama-3.2-1B &  FL most harmful $\lambda=.75$ & {\cellcolor[HTML]{E2DFEE}} \color[HTML]{000000} -18.01 dB \\
Llama-3.2-1B &  FL most helpful $\lambda=.5$ & {\cellcolor[HTML]{E2DFEE}} \color[HTML]{000000} -17.97 dB \\
Llama-3.2-1B &  FL most harmful $\lambda=.5$ & {\cellcolor[HTML]{E2DFEE}} \color[HTML]{000000} -17.92 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{E1DFED}} \color[HTML]{000000} -17.81 dB \\
Llama-3.2-1B &  FL most harmful $\lambda=1$ & {\cellcolor[HTML]{E1DFED}} \color[HTML]{000000} -17.78 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{E1DFED}} \color[HTML]{000000} -17.74 dB \\
Llama-3.2-1B &  FL most helpful $\lambda=.25$ & {\cellcolor[HTML]{E1DFED}} \color[HTML]{000000} -17.74 dB \\
Llama-3.2-1B &  FL most harmful $\lambda=1$ & {\cellcolor[HTML]{E0DEED}} \color[HTML]{000000} -17.64 dB \\
Llama-3.2-1B &  FL most helpful $\lambda=.75$ & {\cellcolor[HTML]{E0DEED}} \color[HTML]{000000} -17.55 dB \\
Llama-3.2-1B &  FL most helpful $\lambda=.5$ & {\cellcolor[HTML]{E0DEED}} \color[HTML]{000000} -17.41 dB \\
Llama-3.2-1B &  DIVINE most harmful & {\cellcolor[HTML]{E0DDED}} \color[HTML]{000000} -17.36 dB \\
Llama-3.2-1B &  DIVINE most harmful & {\cellcolor[HTML]{E0DDED}} \color[HTML]{000000} -17.31 dB \\
Llama-3.2-1B &  DIVINE most inf. & {\cellcolor[HTML]{E0DDED}} \color[HTML]{000000} -17.26 dB \\
Llama-3.2-1B &  DIVINE most inf. & {\cellcolor[HTML]{DFDDEC}} \color[HTML]{000000} -17.06 dB \\
Llama-3.2-1B &  FL most helpful $\lambda=.75$ & {\cellcolor[HTML]{DFDDEC}} \color[HTML]{000000} -17.01 dB \\
Llama-3.2-1B &  DIVINE most helpful & {\cellcolor[HTML]{DEDCEC}} \color[HTML]{000000} -16.82 dB \\
Llama-3.2-1B &  FL most helpful $\lambda=1$ & {\cellcolor[HTML]{DEDCEC}} \color[HTML]{000000} -16.68 dB \\
Llama-3.2-1B &  FL most helpful $\lambda=1$ & {\cellcolor[HTML]{DCDAEB}} \color[HTML]{000000} -16.25 dB \\
Llama-3.2-1B &  DIVINE most helpful & {\cellcolor[HTML]{DBDAEB}} \color[HTML]{000000} -16.08 dB \\
Olmo2-1B &  DIVINE most inf. & {\cellcolor[HTML]{D9D8EA}} \color[HTML]{000000} -15.48 dB \\
Olmo2-1B &  DIVINE most harmful & {\cellcolor[HTML]{D8D7E9}} \color[HTML]{000000} -15.15 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{9CB9D9}} \color[HTML]{000000} -3.50 dB \\
Qwen2.5-0.5B &  DIVINE least inf. & {\cellcolor[HTML]{99B8D8}} \color[HTML]{000000} -3.06 dB \\
Qwen2.5-0.5B & random & {\cellcolor[HTML]{99B8D8}} \color[HTML]{000000} -2.99 dB \\
Llama-3.2-1B & random & {\cellcolor[HTML]{96B6D7}} \color[HTML]{000000} -2.39 dB \\
Olmo2-1B &  DIVINE least inf. & {\cellcolor[HTML]{94B6D7}} \color[HTML]{000000} -2.38 dB \\
Olmo2-1B & random & {\cellcolor[HTML]{94B6D7}} \color[HTML]{000000} -2.37 dB \\
Olmo2-1B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{94B6D7}} \color[HTML]{000000} -2.32 dB \\
Llama-3.2-1B &  DIVINE least inf. & {\cellcolor[HTML]{94B6D7}} \color[HTML]{000000} -2.14 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{93B5D6}} \color[HTML]{000000} -1.96 dB \\
Olmo2-1B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{91B5D6}} \color[HTML]{000000} -1.76 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{8FB4D6}} \color[HTML]{000000} -1.61 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{8FB4D6}} \color[HTML]{000000} -1.58 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{8FB4D6}} \color[HTML]{000000} -1.47 dB \\
Olmo2-1B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{8FB4D6}} \color[HTML]{000000} -1.44 dB \\
Qwen2.5-0.5B & least inf. & {\cellcolor[HTML]{8FB4D6}} \color[HTML]{000000} -1.43 dB \\
Olmo2-1B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{8EB3D5}} \color[HTML]{000000} -1.25 dB \\
Olmo2-1B & least inf. & {\cellcolor[HTML]{8CB3D5}} \color[HTML]{000000} -1.13 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{8CB3D5}} \color[HTML]{000000} -1.03 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{8BB2D4}} \color[HTML]{000000} -0.79 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{89B1D4}} \color[HTML]{000000} -0.60 dB \\
Llama-3.2-1B & least inf. & {\cellcolor[HTML]{89B1D4}} \color[HTML]{000000} -0.52 dB \\
Olmo2-1B & least inf. & {\cellcolor[HTML]{88B1D4}} \color[HTML]{000000} -0.19 dB \\
Olmo2-1B &  DIVINE least inf. & {\cellcolor[HTML]{88B1D4}} \color[HTML]{000000} -0.19 dB \\
Olmo2-1B & least inf. & {\cellcolor[HTML]{88B1D4}} \color[HTML]{000000} -0.19 dB \\
Olmo2-1B &  DIVINE least inf. & {\cellcolor[HTML]{88B1D4}} \color[HTML]{000000} -0.19 dB \\
Olmo2-1B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{88B1D4}} \color[HTML]{000000} -0.18 dB \\
Olmo2-1B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{88B1D4}} \color[HTML]{000000} -0.18 dB \\
Olmo2-1B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{88B1D4}} \color[HTML]{000000} -0.18 dB \\
Olmo2-1B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{88B1D4}} \color[HTML]{000000} -0.18 dB \\
Olmo2-1B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{88B1D4}} \color[HTML]{000000} -0.18 dB \\
Olmo2-1B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{88B1D4}} \color[HTML]{000000} -0.18 dB \\
Olmo2-1B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{88B1D4}} \color[HTML]{000000} -0.18 dB \\
Olmo2-1B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{88B1D4}} \color[HTML]{000000} -0.18 dB \\
Qwen2.5-0.5B &  DIVINE least inf. & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.15 dB \\
Qwen2.5-0.5B & least inf. & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.14 dB \\
Qwen2.5-0.5B &  DIVINE least inf. & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.14 dB \\
Qwen2.5-0.5B & least inf. & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.14 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.13 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.13 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.13 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.13 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.13 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.13 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.13 dB \\
Qwen2.5-0.5B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.13 dB \\
Llama-3.2-1B &  DIVINE least inf. & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.10 dB \\
Llama-3.2-1B & least inf. & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.10 dB \\
Llama-3.2-1B &  DIVINE least inf. & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.10 dB \\
Llama-3.2-1B & least inf. & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.10 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.09 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.09 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.09 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.09 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.08 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=1$ & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.08 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.08 dB \\
Llama-3.2-1B &  FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{86B0D3}} \color[HTML]{000000} -0.08 dB \\
Olmo2-1B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{2987BC}} \color[HTML]{F1F1F1} 12.78 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{167BB6}} \color[HTML]{F1F1F1} 15.65 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=1$ & {\cellcolor[HTML]{0F76B3}} \color[HTML]{F1F1F1} 17.05 dB \\
Olmo2-1B &  DIVINE most inf. & {\cellcolor[HTML]{056BA9}} \color[HTML]{F1F1F1} 20.23 dB \\
Olmo2-1B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{0568A3}} \color[HTML]{F1F1F1} 21.46 dB \\
Olmo2-1B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{0568A3}} \color[HTML]{F1F1F1} 21.46 dB \\
Qwen2.5-0.5B &  AIDE & {\cellcolor[HTML]{0567A2}} \color[HTML]{F1F1F1} 21.62 dB \\
Olmo2-1B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{0567A2}} \color[HTML]{F1F1F1} 21.65 dB \\
Qwen2.5-0.5B & most inf. & {\cellcolor[HTML]{0567A2}} \color[HTML]{F1F1F1} 21.69 dB \\
Olmo2-1B &  AIDE & {\cellcolor[HTML]{0567A1}} \color[HTML]{F1F1F1} 21.86 dB \\
Olmo2-1B & most inf. & {\cellcolor[HTML]{0567A1}} \color[HTML]{F1F1F1} 21.91 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{0566A0}} \color[HTML]{F1F1F1} 22.01 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{05659F}} \color[HTML]{F1F1F1} 22.42 dB \\
Llama-3.2-1B &  DIVINE most inf. & {\cellcolor[HTML]{04649E}} \color[HTML]{F1F1F1} 22.50 dB \\
Llama-3.2-1B &  AIDE & {\cellcolor[HTML]{04649E}} \color[HTML]{F1F1F1} 22.68 dB \\
Llama-3.2-1B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{04649D}} \color[HTML]{F1F1F1} 22.87 dB \\
Llama-3.2-1B & most inf. & {\cellcolor[HTML]{04639B}} \color[HTML]{F1F1F1} 22.99 dB \\
Qwen2.5-0.5B &  DIVINE most inf. & {\cellcolor[HTML]{045A8D}} \color[HTML]{F1F1F1} 26.35 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{023A5B}} \color[HTML]{F1F1F1} 33.63 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{023858}} \color[HTML]{F1F1F1} 34.30 dB \\
Qwen2.5-0.5B &  FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{023858}} \color[HTML]{F1F1F1} 34.30 dB \\
\bottomrule
\end{tabular}


==> tables/scoring/pred_gain/full_per_estimator_selection.tex <==
\begin{tabular}{l|l|l}
\toprule
\midrule
most inf. & {\cellcolor[HTML]{FFF7FB}} \color[HTML]{000000} -23.43 dB \\
most harmful & {\cellcolor[HTML]{FEF6FB}} \color[HTML]{000000} -22.92 dB \\
most inf. & {\cellcolor[HTML]{FEF6FA}} \color[HTML]{000000} -22.85 dB \\
most harmful & {\cellcolor[HTML]{FDF5FA}} \color[HTML]{000000} -22.37 dB \\
most helpful & {\cellcolor[HTML]{FDF5FA}} \color[HTML]{000000} -22.20 dB \\
most helpful & {\cellcolor[HTML]{FCF4FA}} \color[HTML]{000000} -21.98 dB \\
 FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{FAF3F9}} \color[HTML]{000000} -21.19 dB \\
 AIDE & {\cellcolor[HTML]{FAF3F9}} \color[HTML]{000000} -21.16 dB \\
 FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{FAF2F8}} \color[HTML]{000000} -21.01 dB \\
 FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{FAF2F8}} \color[HTML]{000000} -20.91 dB \\
 FL most harmful $\lambda=.25$ & {\cellcolor[HTML]{FAF2F8}} \color[HTML]{000000} -20.83 dB \\
 AIDE & {\cellcolor[HTML]{FAF2F8}} \color[HTML]{000000} -20.77 dB \\
 FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{F9F2F8}} \color[HTML]{000000} -20.71 dB \\
 FL most harmful $\lambda=.25$ & {\cellcolor[HTML]{F9F2F8}} \color[HTML]{000000} -20.65 dB \\
 FL most helpful $\lambda=.25$ & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -20.49 dB \\
 FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -20.47 dB \\
 DIVINE most inf. & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -20.45 dB \\
 FL most harmful $\lambda=.5$ & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -20.42 dB \\
 FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -20.33 dB \\
 FL most helpful $\lambda=.5$ & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -20.21 dB \\
 FL most harmful $\lambda=.5$ & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -20.18 dB \\
 DIVINE most harmful & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -20.18 dB \\
 FL most helpful $\lambda=.25$ & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -20.18 dB \\
 FL most harmful $\lambda=.75$ & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -19.97 dB \\
 FL most helpful $\lambda=.5$ & {\cellcolor[HTML]{F7F0F7}} \color[HTML]{000000} -19.96 dB \\
 FL most helpful $\lambda=.75$ & {\cellcolor[HTML]{F7F0F7}} \color[HTML]{000000} -19.65 dB \\
 FL most inf. $\lambda=1$ & {\cellcolor[HTML]{F7F0F7}} \color[HTML]{000000} -19.65 dB \\
 FL most inf. $\lambda=1$ & {\cellcolor[HTML]{F7F0F7}} \color[HTML]{000000} -19.59 dB \\
 DIVINE most helpful & {\cellcolor[HTML]{F7F0F7}} \color[HTML]{000000} -19.56 dB \\
 FL most helpful $\lambda=.75$ & {\cellcolor[HTML]{F7F0F7}} \color[HTML]{000000} -19.51 dB \\
 FL most harmful $\lambda=.75$ & {\cellcolor[HTML]{F6EFF7}} \color[HTML]{000000} -19.35 dB \\
 DIVINE most helpful & {\cellcolor[HTML]{F6EFF7}} \color[HTML]{000000} -19.33 dB \\
 FL most harmful $\lambda=1$ & {\cellcolor[HTML]{F5EFF6}} \color[HTML]{000000} -19.14 dB \\
 DIVINE most inf. & {\cellcolor[HTML]{F5EFF6}} \color[HTML]{000000} -18.98 dB \\
 FL most harmful $\lambda=1$ & {\cellcolor[HTML]{F4EEF6}} \color[HTML]{000000} -18.54 dB \\
 FL most helpful $\lambda=1$ & {\cellcolor[HTML]{F4EDF6}} \color[HTML]{000000} -18.28 dB \\
 FL most helpful $\lambda=1$ & {\cellcolor[HTML]{F4EDF6}} \color[HTML]{000000} -18.26 dB \\
 DIVINE most harmful & {\cellcolor[HTML]{F3EDF5}} \color[HTML]{000000} -18.06 dB \\
random & {\cellcolor[HTML]{C0C9E2}} \color[HTML]{000000} -2.98 dB \\
 FL least inf. $\lambda=1$ & {\cellcolor[HTML]{BFC9E1}} \color[HTML]{000000} -2.84 dB \\
 DIVINE least inf. & {\cellcolor[HTML]{BBC7E0}} \color[HTML]{000000} -1.86 dB \\
 FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{B7C5DF}} \color[HTML]{000000} -1.27 dB \\
 FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{B7C5DF}} \color[HTML]{000000} -1.04 dB \\
 FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{B5C4DF}} \color[HTML]{000000} -0.92 dB \\
least inf. & {\cellcolor[HTML]{B5C4DF}} \color[HTML]{000000} -0.87 dB \\
 DIVINE least inf. & {\cellcolor[HTML]{B1C2DE}} \color[HTML]{000000} -0.15 dB \\
least inf. & {\cellcolor[HTML]{B1C2DE}} \color[HTML]{000000} -0.15 dB \\
 DIVINE least inf. & {\cellcolor[HTML]{B1C2DE}} \color[HTML]{000000} -0.14 dB \\
least inf. & {\cellcolor[HTML]{B1C2DE}} \color[HTML]{000000} -0.14 dB \\
 FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{B1C2DE}} \color[HTML]{000000} -0.13 dB \\
 FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{B1C2DE}} \color[HTML]{000000} -0.13 dB \\
 FL least inf. $\lambda=1$ & {\cellcolor[HTML]{B1C2DE}} \color[HTML]{000000} -0.13 dB \\
 FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{B1C2DE}} \color[HTML]{000000} -0.13 dB \\
 FL least inf. $\lambda=1$ & {\cellcolor[HTML]{B1C2DE}} \color[HTML]{000000} -0.13 dB \\
 FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{B1C2DE}} \color[HTML]{000000} -0.13 dB \\
 FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{B1C2DE}} \color[HTML]{000000} -0.13 dB \\
 FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{B1C2DE}} \color[HTML]{000000} -0.13 dB \\
 FL most inf. $\lambda=1$ & {\cellcolor[HTML]{509AC6}} \color[HTML]{F1F1F1} 15.72 dB \\
most inf. & {\cellcolor[HTML]{0872B1}} \color[HTML]{F1F1F1} 27.14 dB \\
 AIDE & {\cellcolor[HTML]{0872B1}} \color[HTML]{F1F1F1} 27.22 dB \\
 DIVINE most inf. & {\cellcolor[HTML]{056EAD}} \color[HTML]{F1F1F1} 28.49 dB \\
 FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{056BA9}} \color[HTML]{F1F1F1} 29.51 dB \\
 FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{056BA7}} \color[HTML]{F1F1F1} 29.70 dB \\
 FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{056BA7}} \color[HTML]{F1F1F1} 29.73 dB \\
Test instance & {\cellcolor[HTML]{023858}} \color[HTML]{F1F1F1} 44.91 dB \\
Test instance & {\cellcolor[HTML]{023858}} \color[HTML]{F1F1F1} 44.91 dB \\
Test instance & {\cellcolor[HTML]{023858}} \color[HTML]{F1F1F1} 44.91 dB \\
\bottomrule
\end{tabular}


==> tables/scoring/pred_gain/full_per_estimator_selection_k_10.tex <==
\begin{tabular}{l|l|l}
\toprule
\midrule
most inf. & {\cellcolor[HTML]{FFF7FB}} \color[HTML]{000000} -22.87 dB \\
most harmful & {\cellcolor[HTML]{FEF6FB}} \color[HTML]{000000} -22.50 dB \\
most inf. & {\cellcolor[HTML]{FEF6FA}} \color[HTML]{000000} -22.28 dB \\
most helpful & {\cellcolor[HTML]{FCF4FA}} \color[HTML]{000000} -21.81 dB \\
most harmful & {\cellcolor[HTML]{FCF4FA}} \color[HTML]{000000} -21.79 dB \\
most helpful & {\cellcolor[HTML]{FBF4F9}} \color[HTML]{000000} -21.52 dB \\
 AIDE & {\cellcolor[HTML]{F9F2F8}} \color[HTML]{000000} -20.70 dB \\
 FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{F9F2F8}} \color[HTML]{000000} -20.65 dB \\
 FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -20.56 dB \\
 AIDE & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -20.39 dB \\
 FL most harmful $\lambda=.25$ & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -20.34 dB \\
 FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -20.26 dB \\
 FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{F8F1F8}} \color[HTML]{000000} -20.21 dB \\
 FL most harmful $\lambda=.25$ & {\cellcolor[HTML]{F7F0F7}} \color[HTML]{000000} -20.16 dB \\
 FL most helpful $\lambda=.25$ & {\cellcolor[HTML]{F7F0F7}} \color[HTML]{000000} -20.09 dB \\
 FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{F7F0F7}} \color[HTML]{000000} -19.99 dB \\
 FL most harmful $\lambda=.5$ & {\cellcolor[HTML]{F7F0F7}} \color[HTML]{000000} -19.94 dB \\
 FL most helpful $\lambda=.5$ & {\cellcolor[HTML]{F7F0F7}} \color[HTML]{000000} -19.78 dB \\
 FL most helpful $\lambda=.25$ & {\cellcolor[HTML]{F6EFF7}} \color[HTML]{000000} -19.75 dB \\
 FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{F6EFF7}} \color[HTML]{000000} -19.64 dB \\
 DIVINE most inf. & {\cellcolor[HTML]{F6EFF7}} \color[HTML]{000000} -19.63 dB \\
 FL most harmful $\lambda=.75$ & {\cellcolor[HTML]{F6EFF7}} \color[HTML]{000000} -19.63 dB \\
 FL most inf. $\lambda=1$ & {\cellcolor[HTML]{F5EFF6}} \color[HTML]{000000} -19.54 dB \\
 FL most helpful $\lambda=.5$ & {\cellcolor[HTML]{F5EFF6}} \color[HTML]{000000} -19.49 dB \\
 DIVINE most harmful & {\cellcolor[HTML]{F5EFF6}} \color[HTML]{000000} -19.38 dB \\
 FL most harmful $\lambda=.5$ & {\cellcolor[HTML]{F5EEF6}} \color[HTML]{000000} -19.30 dB \\
 FL most inf. $\lambda=1$ & {\cellcolor[HTML]{F5EEF6}} \color[HTML]{000000} -19.28 dB \\
 FL most harmful $\lambda=.75$ & {\cellcolor[HTML]{F5EEF6}} \color[HTML]{000000} -19.25 dB \\
 FL most helpful $\lambda=.75$ & {\cellcolor[HTML]{F5EEF6}} \color[HTML]{000000} -19.22 dB \\
 FL most helpful $\lambda=.75$ & {\cellcolor[HTML]{F4EEF6}} \color[HTML]{000000} -19.13 dB \\
 FL most harmful $\lambda=1$ & {\cellcolor[HTML]{F4EEF6}} \color[HTML]{000000} -19.07 dB \\
 FL most harmful $\lambda=1$ & {\cellcolor[HTML]{F4EDF6}} \color[HTML]{000000} -18.91 dB \\
 DIVINE most helpful & {\cellcolor[HTML]{F4EDF6}} \color[HTML]{000000} -18.80 dB \\
 DIVINE most helpful & {\cellcolor[HTML]{F3EDF5}} \color[HTML]{000000} -18.69 dB \\
 FL most helpful $\lambda=1$ & {\cellcolor[HTML]{F2ECF5}} \color[HTML]{000000} -18.42 dB \\
 FL most helpful $\lambda=1$ & {\cellcolor[HTML]{F2ECF5}} \color[HTML]{000000} -18.23 dB \\
 DIVINE most inf. & {\cellcolor[HTML]{F0EAF4}} \color[HTML]{000000} -17.31 dB \\
 DIVINE most harmful & {\cellcolor[HTML]{EEE9F3}} \color[HTML]{000000} -17.09 dB \\
random & {\cellcolor[HTML]{A2BCDA}} \color[HTML]{000000} -2.57 dB \\
 DIVINE least inf. & {\cellcolor[HTML]{A2BCDA}} \color[HTML]{000000} -2.51 dB \\
 FL least inf. $\lambda=1$ & {\cellcolor[HTML]{A1BBDA}} \color[HTML]{000000} -2.41 dB \\
 FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{9AB8D8}} \color[HTML]{000000} -1.57 dB \\
 FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{99B8D8}} \color[HTML]{000000} -1.25 dB \\
 FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{97B7D7}} \color[HTML]{000000} -1.09 dB \\
least inf. & {\cellcolor[HTML]{97B7D7}} \color[HTML]{000000} -1.01 dB \\
 DIVINE least inf. & {\cellcolor[HTML]{8FB4D6}} \color[HTML]{000000} -0.15 dB \\
least inf. & {\cellcolor[HTML]{8FB4D6}} \color[HTML]{000000} -0.14 dB \\
 DIVINE least inf. & {\cellcolor[HTML]{8FB4D6}} \color[HTML]{000000} -0.14 dB \\
least inf. & {\cellcolor[HTML]{8FB4D6}} \color[HTML]{000000} -0.14 dB \\
 FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{8FB4D6}} \color[HTML]{000000} -0.13 dB \\
 FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{8FB4D6}} \color[HTML]{000000} -0.13 dB \\
 FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{8FB4D6}} \color[HTML]{000000} -0.13 dB \\
 FL least inf. $\lambda=1$ & {\cellcolor[HTML]{8FB4D6}} \color[HTML]{000000} -0.13 dB \\
 FL least inf. $\lambda=1$ & {\cellcolor[HTML]{8FB4D6}} \color[HTML]{000000} -0.13 dB \\
 FL least inf. $\lambda=.75$ & {\cellcolor[HTML]{8FB4D6}} \color[HTML]{000000} -0.13 dB \\
 FL least inf. $\lambda=.5$ & {\cellcolor[HTML]{8FB4D6}} \color[HTML]{000000} -0.13 dB \\
 FL least inf. $\lambda=.25$ & {\cellcolor[HTML]{8FB4D6}} \color[HTML]{000000} -0.13 dB \\
 FL most inf. $\lambda=1$ & {\cellcolor[HTML]{0F76B3}} \color[HTML]{F1F1F1} 15.50 dB \\
 AIDE & {\cellcolor[HTML]{045E94}} \color[HTML]{F1F1F1} 22.08 dB \\
most inf. & {\cellcolor[HTML]{045E93}} \color[HTML]{F1F1F1} 22.24 dB \\
 DIVINE most inf. & {\cellcolor[HTML]{04588A}} \color[HTML]{F1F1F1} 23.77 dB \\
 FL most inf. $\lambda=.25$ & {\cellcolor[HTML]{023A5B}} \color[HTML]{F1F1F1} 29.44 dB \\
 FL most inf. $\lambda=.75$ & {\cellcolor[HTML]{023858}} \color[HTML]{F1F1F1} 29.99 dB \\
 FL most inf. $\lambda=.5$ & {\cellcolor[HTML]{023858}} \color[HTML]{F1F1F1} 30.00 dB \\
\bottomrule
\end{tabular}


==> tables/scoring/pred_gain_ratio/pred_gain_reduction_BM25Estimator.tex <==
\begin{tabular}{l|l|l}
\toprule
\midrule
Qwen2.5-0.5B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} -18.27 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{E6E5F1}} \color[HTML]{000000} -12.79 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{D6D6E9}} \color[HTML]{000000} -10.00 dB \\
Olmo2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{CFD0E6}} \color[HTML]{000000} -9.14 dB \\
Olmo2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{CACAE3}} \color[HTML]{000000} -8.42 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{C0C1DE}} \color[HTML]{000000} -7.24 dB \\
Olmo2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{BDBEDC}} \color[HTML]{000000} -6.73 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{B7B7D9}} \color[HTML]{000000} -6.04 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{B6B6D8}} \color[HTML]{000000} -5.94 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{B4B4D7}} \color[HTML]{000000} -5.62 dB \\
Olmo2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{B3B3D6}} \color[HTML]{000000} -5.53 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{AEADD3}} \color[HTML]{000000} -4.91 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{A8A6CF}} \color[HTML]{F1F1F1} -4.14 dB \\
Olmo2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{A8A6CF}} \color[HTML]{F1F1F1} -4.08 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{9E9BC8}} \color[HTML]{F1F1F1} -2.91 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{9C98C7}} \color[HTML]{F1F1F1} -2.47 dB \\
Qwen2.5-0.5B & 25 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{9B97C6}} \color[HTML]{F1F1F1} -2.37 dB \\
Olmo2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{9995C6}} \color[HTML]{F1F1F1} -2.20 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{9894C5}} \color[HTML]{F1F1F1} -2.08 dB \\
Llama-3.2-1B & 5 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{9793C5}} \color[HTML]{F1F1F1} -1.90 dB \\
Qwen2.5-0.5B & 25 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{9692C4}} \color[HTML]{F1F1F1} -1.86 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{9692C4}} \color[HTML]{F1F1F1} -1.76 dB \\
Olmo2-1B & 10 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{9591C4}} \color[HTML]{F1F1F1} -1.68 dB \\
Qwen2.5-0.5B & 5 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{9591C4}} \color[HTML]{F1F1F1} -1.64 dB \\
Qwen2.5-0.5B & 10 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{9591C4}} \color[HTML]{F1F1F1} -1.63 dB \\
Llama-3.2-1B & 10 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{9591C4}} \color[HTML]{F1F1F1} -1.63 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{928FC3}} \color[HTML]{F1F1F1} -1.34 dB \\
Olmo2-1B & 25 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{928FC3}} \color[HTML]{F1F1F1} -1.33 dB \\
Olmo2-1B & 10 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{918EC2}} \color[HTML]{F1F1F1} -1.25 dB \\
Olmo2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{918EC2}} \color[HTML]{F1F1F1} -1.19 dB \\
Olmo2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{918EC2}} \color[HTML]{F1F1F1} -1.19 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{908DC2}} \color[HTML]{F1F1F1} -1.09 dB \\
Olmo2-1B & 5 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{908DC2}} \color[HTML]{F1F1F1} -1.09 dB \\
Olmo2-1B & 5 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{908DC2}} \color[HTML]{F1F1F1} -1.07 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{8F8CC1}} \color[HTML]{F1F1F1} -0.98 dB \\
Olmo2-1B & 25 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{8F8CC1}} \color[HTML]{F1F1F1} -0.97 dB \\
Llama-3.2-1B & 25 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{8F8CC1}} \color[HTML]{F1F1F1} -0.94 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{8E8BC1}} \color[HTML]{F1F1F1} -0.83 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{8E8AC0}} \color[HTML]{F1F1F1} -0.69 dB \\
Olmo2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{8D89C0}} \color[HTML]{F1F1F1} -0.64 dB \\
Olmo2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{8D89C0}} \color[HTML]{F1F1F1} -0.63 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{8D89C0}} \color[HTML]{F1F1F1} -0.62 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{8D89C0}} \color[HTML]{F1F1F1} -0.58 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{8C88BF}} \color[HTML]{F1F1F1} -0.53 dB \\
Olmo2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{8C88BF}} \color[HTML]{F1F1F1} -0.52 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{8C88BF}} \color[HTML]{F1F1F1} -0.52 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{8C88BF}} \color[HTML]{F1F1F1} -0.50 dB \\
Llama-3.2-1B & 10 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{8C88BF}} \color[HTML]{F1F1F1} -0.49 dB \\
Olmo2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{8C88BF}} \color[HTML]{F1F1F1} -0.47 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{8C88BF}} \color[HTML]{F1F1F1} -0.46 dB \\
Olmo2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{8C88BF}} \color[HTML]{F1F1F1} -0.46 dB \\
Olmo2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{8C88BF}} \color[HTML]{F1F1F1} -0.45 dB \\
Llama-3.2-1B & 25 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{8C88BF}} \color[HTML]{F1F1F1} -0.45 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{8B87BF}} \color[HTML]{F1F1F1} -0.38 dB \\
Llama-3.2-1B & 10 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{8B87BF}} \color[HTML]{F1F1F1} -0.31 dB \\
Olmo2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{8B87BF}} \color[HTML]{F1F1F1} -0.31 dB \\
Olmo2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{8A86BF}} \color[HTML]{F1F1F1} -0.28 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{8A86BF}} \color[HTML]{F1F1F1} -0.27 dB \\
Olmo2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{8A86BF}} \color[HTML]{F1F1F1} -0.27 dB \\
Olmo2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{8A86BF}} \color[HTML]{F1F1F1} -0.26 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{8A86BF}} \color[HTML]{F1F1F1} -0.20 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{8A86BF}} \color[HTML]{F1F1F1} -0.19 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{8986BE}} \color[HTML]{F1F1F1} -0.16 dB \\
Olmo2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{8986BE}} \color[HTML]{F1F1F1} -0.14 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{8986BE}} \color[HTML]{F1F1F1} -0.14 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{8986BE}} \color[HTML]{F1F1F1} -0.14 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{8986BE}} \color[HTML]{F1F1F1} -0.13 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{8986BE}} \color[HTML]{F1F1F1} -0.13 dB \\
Olmo2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{8986BE}} \color[HTML]{F1F1F1} -0.11 dB \\
Olmo2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{8986BE}} \color[HTML]{F1F1F1} -0.10 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{8986BE}} \color[HTML]{F1F1F1} -0.09 dB \\
Olmo2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{8986BE}} \color[HTML]{F1F1F1} -0.08 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{8986BE}} \color[HTML]{F1F1F1} -0.07 dB \\
Qwen2.5-0.5B & 10 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{8986BE}} \color[HTML]{F1F1F1} -0.07 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{8986BE}} \color[HTML]{F1F1F1} -0.06 dB \\
Olmo2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{8986BE}} \color[HTML]{F1F1F1} -0.06 dB \\
Olmo2-1B & 10 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.05 dB \\
Qwen2.5-0.5B & 25 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.05 dB \\
Llama-3.2-1B & 25 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.05 dB \\
Olmo2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.04 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.04 dB \\
Olmo2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.03 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.03 dB \\
Olmo2-1B & 25 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.02 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.01 dB \\
Olmo2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.01 dB \\
Olmo2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.01 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.01 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.00 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.00 dB \\
Olmo2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.00 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.00 dB \\
Olmo2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.00 dB \\
Olmo2-1B & 1 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} -0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Olmo2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Llama-3.2-1B & 1 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Olmo2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Olmo2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Olmo2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Olmo2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Olmo2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Olmo2-1B & 1 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Qwen2.5-0.5B & 1 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Llama-3.2-1B & 1 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Olmo2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Olmo2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Qwen2.5-0.5B & 1 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Olmo2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Llama-3.2-1B & 1 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Olmo2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.00 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.01 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.05 dB \\
Qwen2.5-0.5B & 5 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.05 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.06 dB \\
Qwen2.5-0.5B & 1 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{8885BE}} \color[HTML]{F1F1F1} 0.06 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{8784BD}} \color[HTML]{F1F1F1} 0.07 dB \\
Olmo2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{8784BD}} \color[HTML]{F1F1F1} 0.08 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{8784BD}} \color[HTML]{F1F1F1} 0.15 dB \\
Llama-3.2-1B & 5 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{8784BD}} \color[HTML]{F1F1F1} 0.18 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{8582BC}} \color[HTML]{F1F1F1} 0.33 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{8582BC}} \color[HTML]{F1F1F1} 0.38 dB \\
Olmo2-1B & 5 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{7F7BB9}} \color[HTML]{F1F1F1} 1.20 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{7E79B8}} \color[HTML]{F1F1F1} 1.37 dB \\
Olmo2-1B & 1 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{7D78B7}} \color[HTML]{F1F1F1} 1.41 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{7D78B7}} \color[HTML]{F1F1F1} 1.49 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{776AB0}} \color[HTML]{F1F1F1} 2.63 dB \\
Qwen2.5-0.5B & 10 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{6B53A4}} \color[HTML]{F1F1F1} 4.66 dB \\
Llama-3.2-1B & 5 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{5B3495}} \color[HTML]{F1F1F1} 7.43 dB \\
Qwen2.5-0.5B & 5 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{51228D}} \color[HTML]{F1F1F1} 9.20 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{460C83}} \color[HTML]{F1F1F1} 11.38 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{460C83}} \color[HTML]{F1F1F1} 11.40 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{450B82}} \color[HTML]{F1F1F1} 11.42 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{420680}} \color[HTML]{F1F1F1} 11.94 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{3F007D}} \color[HTML]{F1F1F1} 12.61 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{3F007D}} \color[HTML]{F1F1F1} 12.61 dB \\
\bottomrule
\end{tabular}


==> tables/scoring/pred_gain_ratio/pred_gain_reduction_DataInfEstimator.tex <==
\begin{tabular}{l|l|l}
\toprule
\midrule
Llama-3.2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} -0.04 dB \\
Qwen2.5-0.5B & 25 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} -0.00 dB \\
Llama-3.2-1B & 10 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} -0.00 dB \\
Qwen2.5-0.5B & 10 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} -0.00 dB \\
Llama-3.2-1B & 25 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} -0.00 dB \\
Qwen2.5-0.5B & 5 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} -0.00 dB \\
Olmo2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} -0.00 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 1 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 1 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 1 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 1 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 1 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 1 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 1 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 1 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 1 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 1 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 1 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 1 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 5 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 10 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 25 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 5 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Olmo2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Olmo2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Olmo2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Olmo2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Olmo2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Olmo2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Olmo2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Olmo2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Olmo2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Olmo2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Olmo2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Olmo2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Olmo2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Olmo2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Olmo2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Olmo2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{FBFAFC}} \color[HTML]{000000} 0.09 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{FAF8FB}} \color[HTML]{000000} 0.32 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{F9F8FB}} \color[HTML]{000000} 0.33 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{F9F8FB}} \color[HTML]{000000} 0.37 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{F8F7FB}} \color[HTML]{000000} 0.46 dB \\
Llama-3.2-1B & 25 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{F8F7FB}} \color[HTML]{000000} 0.48 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{F8F6FA}} \color[HTML]{000000} 0.55 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{F7F6FA}} \color[HTML]{000000} 0.60 dB \\
Llama-3.2-1B & 10 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{F7F6FA}} \color[HTML]{000000} 0.62 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{F7F5FA}} \color[HTML]{000000} 0.65 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{F7F5FA}} \color[HTML]{000000} 0.67 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{F6F4F9}} \color[HTML]{000000} 0.79 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{F4F3F8}} \color[HTML]{000000} 1.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{F4F2F8}} \color[HTML]{000000} 1.04 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{F4F2F8}} \color[HTML]{000000} 1.04 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{F3F1F7}} \color[HTML]{000000} 1.18 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{F2F0F7}} \color[HTML]{000000} 1.23 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{F2F0F7}} \color[HTML]{000000} 1.27 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{F1F0F6}} \color[HTML]{000000} 1.32 dB \\
Llama-3.2-1B & 5 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{F1F0F6}} \color[HTML]{000000} 1.34 dB \\
Qwen2.5-0.5B & 25 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{F1F0F6}} \color[HTML]{000000} 1.36 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{F1EFF6}} \color[HTML]{000000} 1.37 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{F1EFF6}} \color[HTML]{000000} 1.42 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{F1EFF6}} \color[HTML]{000000} 1.43 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{F0EEF6}} \color[HTML]{000000} 1.49 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{F0EEF5}} \color[HTML]{000000} 1.55 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{EFEDF5}} \color[HTML]{000000} 1.59 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{EFEDF5}} \color[HTML]{000000} 1.60 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{EFEDF5}} \color[HTML]{000000} 1.62 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{EFEDF5}} \color[HTML]{000000} 1.64 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{EFEDF5}} \color[HTML]{000000} 1.65 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{EEECF5}} \color[HTML]{000000} 1.69 dB \\
Olmo2-1B & 25 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{EEECF5}} \color[HTML]{000000} 1.69 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{EEECF5}} \color[HTML]{000000} 1.73 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{ECEBF4}} \color[HTML]{000000} 1.87 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{ECEAF3}} \color[HTML]{000000} 1.90 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{EBE9F3}} \color[HTML]{000000} 1.95 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{EBE9F3}} \color[HTML]{000000} 1.97 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{EBE9F3}} \color[HTML]{000000} 1.97 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{EAE9F3}} \color[HTML]{000000} 2.02 dB \\
Llama-3.2-1B & 5 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{EAE9F3}} \color[HTML]{000000} 2.03 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{EAE8F2}} \color[HTML]{000000} 2.08 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{E9E8F2}} \color[HTML]{000000} 2.10 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{E9E8F2}} \color[HTML]{000000} 2.13 dB \\
Qwen2.5-0.5B & 5 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{E8E7F2}} \color[HTML]{000000} 2.17 dB \\
Llama-3.2-1B & 25 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{E7E6F1}} \color[HTML]{000000} 2.25 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{E7E6F1}} \color[HTML]{000000} 2.26 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{E6E5F1}} \color[HTML]{000000} 2.31 dB \\
Qwen2.5-0.5B & 5 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{E6E5F1}} \color[HTML]{000000} 2.38 dB \\
Llama-3.2-1B & 5 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{E6E5F1}} \color[HTML]{000000} 2.39 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{E5E4F0}} \color[HTML]{000000} 2.40 dB \\
Llama-3.2-1B & 25 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{E5E4F0}} \color[HTML]{000000} 2.41 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{E4E3F0}} \color[HTML]{000000} 2.47 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{E4E3F0}} \color[HTML]{000000} 2.49 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{E4E3F0}} \color[HTML]{000000} 2.55 dB \\
Llama-3.2-1B & 5 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{E4E3F0}} \color[HTML]{000000} 2.56 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{E3E2EF}} \color[HTML]{000000} 2.57 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{E3E2EF}} \color[HTML]{000000} 2.58 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{E3E2EF}} \color[HTML]{000000} 2.60 dB \\
Qwen2.5-0.5B & 5 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{E2E2EF}} \color[HTML]{000000} 2.66 dB \\
Llama-3.2-1B & 10 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{E2E2EF}} \color[HTML]{000000} 2.66 dB \\
Llama-3.2-1B & 10 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{E2E1EF}} \color[HTML]{000000} 2.68 dB \\
Qwen2.5-0.5B & 10 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{E2E1EF}} \color[HTML]{000000} 2.69 dB \\
Llama-3.2-1B & 10 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{E2E1EF}} \color[HTML]{000000} 2.69 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{E1E0EE}} \color[HTML]{000000} 2.74 dB \\
Llama-3.2-1B & 25 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{E1E0EE}} \color[HTML]{000000} 2.75 dB \\
Olmo2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{E1E0EE}} \color[HTML]{000000} 2.76 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{E0E0EE}} \color[HTML]{000000} 2.77 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{E0DFEE}} \color[HTML]{000000} 2.83 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{DFDFED}} \color[HTML]{000000} 2.89 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{DEDEED}} \color[HTML]{000000} 2.93 dB \\
Olmo2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{DEDEED}} \color[HTML]{000000} 2.95 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{DEDEED}} \color[HTML]{000000} 2.96 dB \\
Olmo2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{DEDDED}} \color[HTML]{000000} 3.00 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{DEDDED}} \color[HTML]{000000} 3.01 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{DCDCEC}} \color[HTML]{000000} 3.08 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{DCDCEC}} \color[HTML]{000000} 3.11 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{DCDCEC}} \color[HTML]{000000} 3.12 dB \\
Qwen2.5-0.5B & 25 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{DCDCEC}} \color[HTML]{000000} 3.16 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{DCDCEC}} \color[HTML]{000000} 3.17 dB \\
Olmo2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{DADAEB}} \color[HTML]{000000} 3.23 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{DADAEB}} \color[HTML]{000000} 3.24 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{DADAEB}} \color[HTML]{000000} 3.28 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{DADAEB}} \color[HTML]{000000} 3.29 dB \\
Olmo2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{DADAEB}} \color[HTML]{000000} 3.31 dB \\
Olmo2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{DADAEB}} \color[HTML]{000000} 3.33 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{DADAEB}} \color[HTML]{000000} 3.33 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{D9D9EA}} \color[HTML]{000000} 3.35 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{D9D9EA}} \color[HTML]{000000} 3.36 dB \\
Qwen2.5-0.5B & 25 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{D9D9EA}} \color[HTML]{000000} 3.36 dB \\
Qwen2.5-0.5B & 10 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{D9D9EA}} \color[HTML]{000000} 3.37 dB \\
Olmo2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{D8D8EA}} \color[HTML]{000000} 3.42 dB \\
Qwen2.5-0.5B & 25 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{D7D7E9}} \color[HTML]{000000} 3.45 dB \\
Qwen2.5-0.5B & 5 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{D7D7E9}} \color[HTML]{000000} 3.49 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{D6D6E9}} \color[HTML]{000000} 3.49 dB \\
Qwen2.5-0.5B & 10 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{D6D6E9}} \color[HTML]{000000} 3.51 dB \\
Olmo2-1B & 5 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{D6D6E9}} \color[HTML]{000000} 3.53 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{D5D5E9}} \color[HTML]{000000} 3.56 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{D5D5E9}} \color[HTML]{000000} 3.56 dB \\
Olmo2-1B & 10 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{D4D4E8}} \color[HTML]{000000} 3.63 dB \\
Olmo2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{D4D4E8}} \color[HTML]{000000} 3.63 dB \\
Olmo2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{D4D4E8}} \color[HTML]{000000} 3.63 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{D4D4E8}} \color[HTML]{000000} 3.63 dB \\
Olmo2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{D2D2E7}} \color[HTML]{000000} 3.71 dB \\
Qwen2.5-0.5B & 10 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{D1D2E7}} \color[HTML]{000000} 3.75 dB \\
Olmo2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{D1D2E7}} \color[HTML]{000000} 3.77 dB \\
Llama-3.2-1B & 1 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{D1D2E7}} \color[HTML]{000000} 3.78 dB \\
Olmo2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{D0D1E6}} \color[HTML]{000000} 3.81 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{D0D1E6}} \color[HTML]{000000} 3.82 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{CECFE5}} \color[HTML]{000000} 3.93 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{CECFE5}} \color[HTML]{000000} 3.94 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{CECFE5}} \color[HTML]{000000} 3.95 dB \\
Olmo2-1B & 25 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{CBCBE3}} \color[HTML]{000000} 4.13 dB \\
Olmo2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{CACAE3}} \color[HTML]{000000} 4.20 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{C9C9E2}} \color[HTML]{000000} 4.24 dB \\
Olmo2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{C9C9E2}} \color[HTML]{000000} 4.26 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{C9C9E2}} \color[HTML]{000000} 4.26 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{C8C8E2}} \color[HTML]{000000} 4.28 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{C7C8E1}} \color[HTML]{000000} 4.37 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{C6C7E1}} \color[HTML]{000000} 4.39 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{C6C7E1}} \color[HTML]{000000} 4.41 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{C5C6E1}} \color[HTML]{000000} 4.43 dB \\
Olmo2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{C5C6E1}} \color[HTML]{000000} 4.46 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{C3C4E0}} \color[HTML]{000000} 4.55 dB \\
Olmo2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{C0C1DE}} \color[HTML]{000000} 4.69 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{C0C1DE}} \color[HTML]{000000} 4.71 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{BEBFDD}} \color[HTML]{000000} 4.79 dB \\
Olmo2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{BEBFDD}} \color[HTML]{000000} 4.80 dB \\
Olmo2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{BEBFDD}} \color[HTML]{000000} 4.83 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{BEBFDD}} \color[HTML]{000000} 4.83 dB \\
Olmo2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{BDBEDC}} \color[HTML]{000000} 4.94 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{BBBBDB}} \color[HTML]{000000} 5.05 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{BABADB}} \color[HTML]{000000} 5.06 dB \\
Olmo2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{BABADB}} \color[HTML]{000000} 5.08 dB \\
Olmo2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{BABADB}} \color[HTML]{000000} 5.08 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{B5B5D7}} \color[HTML]{000000} 5.33 dB \\
Olmo2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{B2B2D5}} \color[HTML]{000000} 5.51 dB \\
Olmo2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{B1B1D5}} \color[HTML]{000000} 5.52 dB \\
Olmo2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{B1B1D5}} \color[HTML]{000000} 5.56 dB \\
Olmo2-1B & 10 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{B0AFD4}} \color[HTML]{000000} 5.61 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{ACAAD1}} \color[HTML]{000000} 5.84 dB \\
Olmo2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{ABA9D0}} \color[HTML]{000000} 5.89 dB \\
Olmo2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{AAA8D0}} \color[HTML]{000000} 5.94 dB \\
Olmo2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{A4A1CC}} \color[HTML]{F1F1F1} 6.29 dB \\
Olmo2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{A09DCA}} \color[HTML]{F1F1F1} 6.48 dB \\
Olmo2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{9F9CC9}} \color[HTML]{F1F1F1} 6.51 dB \\
Olmo2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{9F9CC9}} \color[HTML]{F1F1F1} 6.52 dB \\
Olmo2-1B & 5 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{9F9CC9}} \color[HTML]{F1F1F1} 6.54 dB \\
Olmo2-1B & 5 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{9C98C7}} \color[HTML]{F1F1F1} 6.73 dB \\
Olmo2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{9A96C6}} \color[HTML]{F1F1F1} 6.84 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{9793C5}} \color[HTML]{F1F1F1} 6.98 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{9793C5}} \color[HTML]{F1F1F1} 6.98 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{9793C5}} \color[HTML]{F1F1F1} 7.01 dB \\
Olmo2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{9390C3}} \color[HTML]{F1F1F1} 7.22 dB \\
Olmo2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{918EC2}} \color[HTML]{F1F1F1} 7.31 dB \\
Olmo2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{918EC2}} \color[HTML]{F1F1F1} 7.31 dB \\
Olmo2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{8D89C0}} \color[HTML]{F1F1F1} 7.56 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{8B87BF}} \color[HTML]{F1F1F1} 7.67 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{8B87BF}} \color[HTML]{F1F1F1} 7.67 dB \\
Olmo2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{8A86BF}} \color[HTML]{F1F1F1} 7.74 dB \\
Olmo2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{8784BD}} \color[HTML]{F1F1F1} 7.89 dB \\
Olmo2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{8784BD}} \color[HTML]{F1F1F1} 7.89 dB \\
Olmo2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{827FBB}} \color[HTML]{F1F1F1} 8.13 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{827FBB}} \color[HTML]{F1F1F1} 8.13 dB \\
Olmo2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{807CBA}} \color[HTML]{F1F1F1} 8.27 dB \\
Olmo2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{807CBA}} \color[HTML]{F1F1F1} 8.29 dB \\
Olmo2-1B & 25 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{7D77B7}} \color[HTML]{F1F1F1} 8.51 dB \\
Qwen2.5-0.5B & 1 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{7B72B4}} \color[HTML]{F1F1F1} 8.66 dB \\
Olmo2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{7A71B4}} \color[HTML]{F1F1F1} 8.68 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{776AB0}} \color[HTML]{F1F1F1} 8.97 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{6E58A7}} \color[HTML]{F1F1F1} 9.63 dB \\
Olmo2-1B & 1 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{6C55A5}} \color[HTML]{F1F1F1} 9.72 dB \\
Olmo2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{6C54A5}} \color[HTML]{F1F1F1} 9.79 dB \\
Olmo2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{6B53A4}} \color[HTML]{F1F1F1} 9.82 dB \\
Olmo2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{6B53A4}} \color[HTML]{F1F1F1} 9.83 dB \\
Olmo2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{6A51A3}} \color[HTML]{F1F1F1} 9.92 dB \\
Olmo2-1B & 25 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{62429C}} \color[HTML]{F1F1F1} 10.50 dB \\
Olmo2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{613F9A}} \color[HTML]{F1F1F1} 10.62 dB \\
Olmo2-1B & 10 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{603E9A}} \color[HTML]{F1F1F1} 10.68 dB \\
Olmo2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{5A3294}} \color[HTML]{F1F1F1} 11.14 dB \\
Olmo2-1B & 5 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{470F84}} \color[HTML]{F1F1F1} 12.59 dB \\
Olmo2-1B & 10 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{3F007D}} \color[HTML]{F1F1F1} 13.24 dB \\
\bottomrule
\end{tabular}


==> tables/scoring/pred_gain_ratio/pred_gain_reduction_LESSEstimator.tex <==
\begin{tabular}{l|l|l}
\toprule
\midrule
Qwen2.5-0.5B & 25 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} -0.00 dB \\
Qwen2.5-0.5B & 10 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} -0.00 dB \\
Llama-3.2-1B & 10 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} -0.00 dB \\
Qwen2.5-0.5B & 5 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} -0.00 dB \\
Llama-3.2-1B & 25 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} -0.00 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 1 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 1 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 1 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 1 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 1 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 1 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 1 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 1 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 1 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 1 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 1 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 1 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 10 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 5 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 5 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Olmo2-1B & 25 by DIVINE from Top-100 least influential (scores closest to zero). & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.00 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Olmo2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Olmo2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Olmo2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Olmo2-1B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Olmo2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Olmo2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Olmo2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Olmo2-1B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.01 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Olmo2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Olmo2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Olmo2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Olmo2-1B & 1 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Olmo2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.75 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Olmo2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.25 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Olmo2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=1.0 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Olmo2-1B & 25 by facility location from Top-100 least influential (scores closest to zero). lambda=0.5 & {\cellcolor[HTML]{FCFBFD}} \color[HTML]{000000} 0.02 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{FAF8FB}} \color[HTML]{000000} 0.28 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{FAF8FB}} \color[HTML]{000000} 0.29 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{F9F8FB}} \color[HTML]{000000} 0.35 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{F9F7FB}} \color[HTML]{000000} 0.41 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{F8F7FB}} \color[HTML]{000000} 0.46 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{F8F7FA}} \color[HTML]{000000} 0.48 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{F8F6FA}} \color[HTML]{000000} 0.54 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{F8F6FA}} \color[HTML]{000000} 0.54 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{F7F6FA}} \color[HTML]{000000} 0.57 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{F7F6FA}} \color[HTML]{000000} 0.60 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{F6F5F9}} \color[HTML]{000000} 0.70 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{F6F5F9}} \color[HTML]{000000} 0.70 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{F5F4F9}} \color[HTML]{000000} 0.78 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{F5F4F9}} \color[HTML]{000000} 0.82 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{F5F3F8}} \color[HTML]{000000} 0.87 dB \\
Llama-3.2-1B & 25 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{F5F3F8}} \color[HTML]{000000} 0.87 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{F5F3F8}} \color[HTML]{000000} 0.89 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{F5F3F8}} \color[HTML]{000000} 0.89 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{F4F2F8}} \color[HTML]{000000} 0.96 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{F4F2F8}} \color[HTML]{000000} 0.98 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{F4F2F8}} \color[HTML]{000000} 0.98 dB \\
Llama-3.2-1B & 5 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{F3F2F8}} \color[HTML]{000000} 1.00 dB \\
Llama-3.2-1B & 10 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{F3F2F8}} \color[HTML]{000000} 1.00 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{F3F2F8}} \color[HTML]{000000} 1.01 dB \\
Llama-3.2-1B & 5 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{F3F1F7}} \color[HTML]{000000} 1.06 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{F2F0F7}} \color[HTML]{000000} 1.13 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{F2F0F7}} \color[HTML]{000000} 1.14 dB \\
Llama-3.2-1B & 5 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{F2F0F7}} \color[HTML]{000000} 1.22 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{F1F0F6}} \color[HTML]{000000} 1.26 dB \\
Olmo2-1B & 25 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{F1EFF6}} \color[HTML]{000000} 1.31 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{F1EFF6}} \color[HTML]{000000} 1.35 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{F1EFF6}} \color[HTML]{000000} 1.36 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{F0EEF6}} \color[HTML]{000000} 1.36 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{F0EEF6}} \color[HTML]{000000} 1.40 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{F0EEF6}} \color[HTML]{000000} 1.41 dB \\
Qwen2.5-0.5B & 25 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{F0EEF5}} \color[HTML]{000000} 1.44 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{F0EEF5}} \color[HTML]{000000} 1.45 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{F0EEF5}} \color[HTML]{000000} 1.45 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{EFEDF5}} \color[HTML]{000000} 1.48 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{EFEDF5}} \color[HTML]{000000} 1.50 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{EEECF5}} \color[HTML]{000000} 1.56 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{EEECF4}} \color[HTML]{000000} 1.63 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{EDEBF4}} \color[HTML]{000000} 1.65 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{ECEBF4}} \color[HTML]{000000} 1.71 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{ECEBF4}} \color[HTML]{000000} 1.74 dB \\
Llama-3.2-1B & 5 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{EBE9F3}} \color[HTML]{000000} 1.83 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{EAE9F3}} \color[HTML]{000000} 1.87 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{E9E8F2}} \color[HTML]{000000} 1.96 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{E8E7F2}} \color[HTML]{000000} 1.99 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{E8E6F2}} \color[HTML]{000000} 2.05 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{E8E6F2}} \color[HTML]{000000} 2.06 dB \\
Llama-3.2-1B & 10 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{E7E6F1}} \color[HTML]{000000} 2.11 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{E7E6F1}} \color[HTML]{000000} 2.12 dB \\
Llama-3.2-1B & 25 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{E6E5F1}} \color[HTML]{000000} 2.16 dB \\
Llama-3.2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{E5E4F0}} \color[HTML]{000000} 2.23 dB \\
Qwen2.5-0.5B & 5 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{E5E4F0}} \color[HTML]{000000} 2.25 dB \\
Llama-3.2-1B & 10 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{E4E3F0}} \color[HTML]{000000} 2.26 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{E4E3F0}} \color[HTML]{000000} 2.33 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{E4E3F0}} \color[HTML]{000000} 2.35 dB \\
Olmo2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{E3E2EF}} \color[HTML]{000000} 2.36 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{E3E2EF}} \color[HTML]{000000} 2.37 dB \\
Qwen2.5-0.5B & 25 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{E3E2EF}} \color[HTML]{000000} 2.37 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{E2E2EF}} \color[HTML]{000000} 2.43 dB \\
Qwen2.5-0.5B & 10 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{E2E2EF}} \color[HTML]{000000} 2.44 dB \\
Llama-3.2-1B & 25 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{E2E1EF}} \color[HTML]{000000} 2.45 dB \\
Olmo2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{E2E1EF}} \color[HTML]{000000} 2.46 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{E0E0EE}} \color[HTML]{000000} 2.57 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{E0E0EE}} \color[HTML]{000000} 2.57 dB \\
Llama-3.2-1B & 25 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{E0DFEE}} \color[HTML]{000000} 2.60 dB \\
Llama-3.2-1B & 10 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{E0DFEE}} \color[HTML]{000000} 2.60 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{E0DFEE}} \color[HTML]{000000} 2.62 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{E0DFEE}} \color[HTML]{000000} 2.62 dB \\
Olmo2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{E0DFEE}} \color[HTML]{000000} 2.63 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{DFDFED}} \color[HTML]{000000} 2.68 dB \\
Qwen2.5-0.5B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{DFDFED}} \color[HTML]{000000} 2.68 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{DEDEED}} \color[HTML]{000000} 2.69 dB \\
Qwen2.5-0.5B & 10 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{DEDEED}} \color[HTML]{000000} 2.70 dB \\
Llama-3.2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{DEDDED}} \color[HTML]{000000} 2.74 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{DEDDED}} \color[HTML]{000000} 2.76 dB \\
Qwen2.5-0.5B & 25 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{DEDDED}} \color[HTML]{000000} 2.77 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{DEDDED}} \color[HTML]{000000} 2.77 dB \\
Qwen2.5-0.5B & 5 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{DEDDED}} \color[HTML]{000000} 2.77 dB \\
Olmo2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{DDDDEC}} \color[HTML]{000000} 2.78 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{DDDDEC}} \color[HTML]{000000} 2.79 dB \\
Qwen2.5-0.5B & 10 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{DCDCEC}} \color[HTML]{000000} 2.90 dB \\
Olmo2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{DCDCEC}} \color[HTML]{000000} 2.91 dB \\
Qwen2.5-0.5B & 25 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{DBDBEC}} \color[HTML]{000000} 2.94 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{DBDBEC}} \color[HTML]{000000} 2.96 dB \\
Olmo2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{DADAEB}} \color[HTML]{000000} 3.04 dB \\
Llama-3.2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{DADAEB}} \color[HTML]{000000} 3.04 dB \\
Olmo2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{D8D8EA}} \color[HTML]{000000} 3.13 dB \\
Olmo2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{D8D8EA}} \color[HTML]{000000} 3.14 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{D6D6E9}} \color[HTML]{000000} 3.24 dB \\
Olmo2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{D6D6E9}} \color[HTML]{000000} 3.24 dB \\
Olmo2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{D6D6E9}} \color[HTML]{000000} 3.25 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{D4D4E8}} \color[HTML]{000000} 3.29 dB \\
Olmo2-1B & 25 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{D4D4E8}} \color[HTML]{000000} 3.31 dB \\
Olmo2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{D4D4E8}} \color[HTML]{000000} 3.31 dB \\
Olmo2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{D4D4E8}} \color[HTML]{000000} 3.34 dB \\
Olmo2-1B & 10 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{D4D4E8}} \color[HTML]{000000} 3.34 dB \\
Qwen2.5-0.5B & 10 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{D3D3E8}} \color[HTML]{000000} 3.35 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{D3D3E8}} \color[HTML]{000000} 3.36 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{D2D2E7}} \color[HTML]{000000} 3.41 dB \\
Olmo2-1B & 5 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{D2D2E7}} \color[HTML]{000000} 3.42 dB \\
Olmo2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{D2D2E7}} \color[HTML]{000000} 3.43 dB \\
Olmo2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{D2D2E7}} \color[HTML]{000000} 3.43 dB \\
Qwen2.5-0.5B & 5 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{D1D2E7}} \color[HTML]{000000} 3.48 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{D0D1E6}} \color[HTML]{000000} 3.52 dB \\
Qwen2.5-0.5B & 5 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{CFD0E6}} \color[HTML]{000000} 3.55 dB \\
Olmo2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{CFD0E6}} \color[HTML]{000000} 3.55 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{CFD0E6}} \color[HTML]{000000} 3.55 dB \\
Olmo2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{CFD0E6}} \color[HTML]{000000} 3.56 dB \\
Olmo2-1B & 10 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{CECFE5}} \color[HTML]{000000} 3.58 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{CECFE5}} \color[HTML]{000000} 3.60 dB \\
Olmo2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{CECFE5}} \color[HTML]{000000} 3.61 dB \\
Olmo2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{CECFE5}} \color[HTML]{000000} 3.61 dB \\
Olmo2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{CECEE5}} \color[HTML]{000000} 3.64 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{CECEE5}} \color[HTML]{000000} 3.66 dB \\
Olmo2-1B & 25 by DIVINE from Top-100 most harmful (most positive scores). & {\cellcolor[HTML]{CDCDE4}} \color[HTML]{000000} 3.67 dB \\
Olmo2-1B & 10 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{CDCDE4}} \color[HTML]{000000} 3.69 dB \\
Olmo2-1B & 10 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{CDCDE4}} \color[HTML]{000000} 3.70 dB \\
Olmo2-1B & 25 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{CDCDE4}} \color[HTML]{000000} 3.71 dB \\
Olmo2-1B & 5 by DIVINE from Top-100 most helpful (most negative scores). & {\cellcolor[HTML]{CCCCE4}} \color[HTML]{000000} 3.76 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{CBCBE3}} \color[HTML]{000000} 3.79 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{CBCBE3}} \color[HTML]{000000} 3.80 dB \\
Olmo2-1B & 25 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{CACAE3}} \color[HTML]{000000} 3.85 dB \\
Olmo2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{C9C9E2}} \color[HTML]{000000} 3.87 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{C9C9E2}} \color[HTML]{000000} 3.88 dB \\
Olmo2-1B & 5 by DIVINE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{C9C9E2}} \color[HTML]{000000} 3.88 dB \\
Olmo2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{C9C9E2}} \color[HTML]{000000} 3.90 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{C8C8E2}} \color[HTML]{000000} 3.92 dB \\
Olmo2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{C8C8E2}} \color[HTML]{000000} 3.92 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{C8C8E2}} \color[HTML]{000000} 3.94 dB \\
Olmo2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{C7C8E1}} \color[HTML]{000000} 3.96 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{C7C8E1}} \color[HTML]{000000} 3.98 dB \\
Olmo2-1B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{C6C7E1}} \color[HTML]{000000} 4.02 dB \\
Olmo2-1B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{C6C7E1}} \color[HTML]{000000} 4.03 dB \\
Olmo2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{C3C4E0}} \color[HTML]{000000} 4.17 dB \\
Llama-3.2-1B & 1 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{C1C2DF}} \color[HTML]{000000} 4.25 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{C1C2DF}} \color[HTML]{000000} 4.26 dB \\
Olmo2-1B & 10 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{BEBFDD}} \color[HTML]{000000} 4.39 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{BEBEDD}} \color[HTML]{000000} 4.47 dB \\
Olmo2-1B & 25 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{BDBEDC}} \color[HTML]{000000} 4.48 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{BBBBDB}} \color[HTML]{000000} 4.56 dB \\
Olmo2-1B & 25 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{BBBBDB}} \color[HTML]{000000} 4.58 dB \\
Olmo2-1B & 5 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{BABADB}} \color[HTML]{000000} 4.65 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{B9B9DA}} \color[HTML]{000000} 4.67 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{B9B9DA}} \color[HTML]{000000} 4.67 dB \\
Olmo2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{B9B9DA}} \color[HTML]{000000} 4.68 dB \\
Olmo2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{B8B8D9}} \color[HTML]{000000} 4.72 dB \\
Olmo2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{B6B6D8}} \color[HTML]{000000} 4.82 dB \\
Qwen2.5-0.5B & 10 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{B5B5D7}} \color[HTML]{000000} 4.86 dB \\
Qwen2.5-0.5B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{B5B5D7}} \color[HTML]{000000} 4.89 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{B0AFD4}} \color[HTML]{000000} 5.12 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{AEADD3}} \color[HTML]{000000} 5.18 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{AEADD3}} \color[HTML]{000000} 5.18 dB \\
Olmo2-1B & 5 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{AEACD2}} \color[HTML]{000000} 5.23 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{ACAAD1}} \color[HTML]{000000} 5.34 dB \\
Olmo2-1B & 5 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{A9A7CF}} \color[HTML]{F1F1F1} 5.47 dB \\
Qwen2.5-0.5B & 1 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{A6A3CD}} \color[HTML]{F1F1F1} 5.62 dB \\
Olmo2-1B & 5 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{A6A3CD}} \color[HTML]{F1F1F1} 5.63 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{A3A0CB}} \color[HTML]{F1F1F1} 5.75 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{A3A0CB}} \color[HTML]{F1F1F1} 5.75 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{A09DCA}} \color[HTML]{F1F1F1} 5.91 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{A09DCA}} \color[HTML]{F1F1F1} 5.91 dB \\
Olmo2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.5 & {\cellcolor[HTML]{9692C4}} \color[HTML]{F1F1F1} 6.44 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{9692C4}} \color[HTML]{F1F1F1} 6.45 dB \\
Olmo2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.25 & {\cellcolor[HTML]{9591C4}} \color[HTML]{F1F1F1} 6.49 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{908DC2}} \color[HTML]{F1F1F1} 6.72 dB \\
Olmo2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=0.75 & {\cellcolor[HTML]{8B87BF}} \color[HTML]{F1F1F1} 7.00 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{8986BE}} \color[HTML]{F1F1F1} 7.08 dB \\
Llama-3.2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{8986BE}} \color[HTML]{F1F1F1} 7.10 dB \\
Qwen2.5-0.5B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{7970B3}} \color[HTML]{F1F1F1} 7.98 dB \\
Olmo2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.5 & {\cellcolor[HTML]{7261AB}} \color[HTML]{F1F1F1} 8.50 dB \\
Olmo2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.25 & {\cellcolor[HTML]{715FAA}} \color[HTML]{F1F1F1} 8.54 dB \\
Olmo2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=0.75 & {\cellcolor[HTML]{6E5AA8}} \color[HTML]{F1F1F1} 8.71 dB \\
Olmo2-1B & 1 by facility location from Top-100 most helpful (most negative scores). lambda=1.0 & {\cellcolor[HTML]{552890}} \color[HTML]{F1F1F1} 10.46 dB \\
Olmo2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.5 & {\cellcolor[HTML]{53258E}} \color[HTML]{F1F1F1} 10.61 dB \\
Olmo2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.25 & {\cellcolor[HTML]{53258E}} \color[HTML]{F1F1F1} 10.61 dB \\
Olmo2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=0.75 & {\cellcolor[HTML]{51218C}} \color[HTML]{F1F1F1} 10.75 dB \\
Olmo2-1B & 1 by AIDE from Top-100 most influential (scores with largest absolute value). & {\cellcolor[HTML]{4C1788}} \color[HTML]{F1F1F1} 11.14 dB \\
Olmo2-1B & 1 by facility location from Top-100 most harmful (most positive scores). lambda=1.0 & {\cellcolor[HTML]{440A82}} \color[HTML]{F1F1F1} 11.64 dB \\
Olmo2-1B & 1 by facility location from Top-100 most influential (scores with largest absolute value). lambda=1.0 & {\cellcolor[HTML]{3F007D}} \color[HTML]{F1F1F1} 12.05 dB \\
\bottomrule
\end{tabular}


==> tables/validation/full/MSECoderProjUSimp.tex <==
\begin{tabular}{llll}
\toprule
 &  &  &  & $\rho(\xi^{{\mathcal{{SR}}}}, \xi^+)$ & $\rho(\xi^{{\mathcal{{SR}}}}, \xi^{JSD})$ \\
train_dataset & train_split & test_dataset & test_split &  &  \\
\midrule
loris3/tulu-3-sft-olmo-2-mixture-0225-sample & train & loris3/tulu-3-sft-olmo-2-mixture-0225-sample & test & {\cellcolor[rgb]{0.922, 0.961, 0.976}} \color{black} 0.093349 & {\cellcolor[rgb]{0.941, 0.969, 0.980}} \color{black} 0.072748 \\
\bottomrule
\end{tabular}


==> tables/validation/full/pred_gain_filtMSECoderProjUSimp.tex <==
\begin{tabular}{llll}
\toprule
 &  &  &  & $\rho(\xi^{{\mathcal{{SR}}}}, \xi^+)$ & $\rho(\xi^{{\mathcal{{SR}}}}, \xi^{JSD})$ \\
train_dataset & train_split & test_dataset & test_split &  &  \\
\midrule
loris3/tulu-3-sft-olmo-2-mixture-0225-sample & train & loris3/tulu-3-sft-olmo-2-mixture-0225-sample & test & {\cellcolor[rgb]{0.537, 0.761, 0.875}} \color{black} 0.575404 & {\cellcolor[rgb]{0.698, 0.843, 0.918}} \color{black} 0.374393 \\
\bottomrule
\end{tabular}


==> tables/validation/per_estimator/pred_gain_filtMSECoderProjUSimp.tex <==
\begin{tabular}{llllllll}
\toprule
 & $\rho(\xi^{{\mathcal{{SR}}}}, \xi^+)$ & $\rho(\xi^{{\mathcal{{SR}}}}, \xi^{JSD})$ \\
Estimator &  &  \\
\midrule
BM25Estimator & {\cellcolor[rgb]{0.592, 0.792, 0.890}} \color{black} 0.504711 & {\cellcolor[rgb]{0.741, 0.867, 0.929}} \color{black} 0.317209 \\
DataInfEstimator & {\cellcolor[rgb]{0.945, 0.969, 0.984}} \color{black} -0.068170 & {\cellcolor[rgb]{0.627, 0.808, 0.898}} \color{black} 0.460028 \\
LESSEstimator & {\cellcolor[rgb]{0.925, 0.961, 0.980}} \color{black} -0.088571 & {\cellcolor[rgb]{0.624, 0.808, 0.898}} \color{black} 0.463996 \\
\bottomrule
\end{tabular}


==> tables/validation/per_strategy/MSECoderProjUSimp.tex <==
\begin{tabular}{llllllll}
\toprule
 &  & $\rho(\xi^{{\mathcal{{SR}}}}, \xi^+)$ & $\rho(\xi^{{\mathcal{{SR}}}}, \xi^{JSD})$ \\
Estimator & cat &  &  \\
\midrule
\multirow[c]{5}{*}{BM25Estimator} & 0.0 & {\cellcolor[rgb]{0.635, 0.812, 0.902}} \color{black} 0.453136 & {\cellcolor[rgb]{0.773, 0.882, 0.937}} \color{black} 0.279474 \\
 & 0.25 & {\cellcolor[rgb]{0.635, 0.812, 0.902}} \color{black} 0.452241 & {\cellcolor[rgb]{0.776, 0.886, 0.937}} \color{black} 0.274084 \\
 & 0.5 & {\cellcolor[rgb]{0.635, 0.812, 0.902}} \color{black} 0.452760 & {\cellcolor[rgb]{0.769, 0.878, 0.937}} \color{black} 0.287540 \\
 & 0.75 & {\cellcolor[rgb]{0.643, 0.816, 0.902}} \color{black} 0.441320 & {\cellcolor[rgb]{0.773, 0.882, 0.937}} \color{black} 0.281763 \\
 & 1.0 & {\cellcolor[rgb]{0.780, 0.886, 0.937}} \color{black} 0.273096 & {\cellcolor[rgb]{0.737, 0.867, 0.929}} \color{black} 0.322542 \\
\multirow[c]{5}{*}{DataInfEstimator} & 0.0 & {\cellcolor[rgb]{0.875, 0.937, 0.965}} \color{black} 0.152344 & {\cellcolor[rgb]{0.882, 0.937, 0.965}} \color{black} -0.145919 \\
 & 0.25 & {\cellcolor[rgb]{0.949, 0.973, 0.984}} \color{black} 0.061095 & {\cellcolor[rgb]{0.859, 0.925, 0.961}} \color{black} -0.171511 \\
 & 0.5 & {\cellcolor[rgb]{0.761, 0.878, 0.933}} \color{black} 0.293571 & {\cellcolor[rgb]{0.820, 0.906, 0.949}} \color{black} -0.220772 \\
 & 0.75 & {\cellcolor[rgb]{0.871, 0.933, 0.965}} \color{black} 0.160814 & {\cellcolor[rgb]{0.710, 0.851, 0.922}} \color{black} -0.356370 \\
 & 1.0 & {\cellcolor[rgb]{0.820, 0.906, 0.949}} \color{black} 0.223581 & {\cellcolor[rgb]{0.776, 0.886, 0.937}} \color{black} -0.274671 \\
\multirow[c]{5}{*}{LESSEstimator} & 0.0 & {\cellcolor[rgb]{0.980, 0.988, 0.992}} \color{black} -0.023850 & {\cellcolor[rgb]{0.820, 0.906, 0.949}} \color{black} 0.221928 \\
 & 0.25 & {\cellcolor[rgb]{0.835, 0.914, 0.953}} \color{black} 0.204794 & {\cellcolor[rgb]{0.749, 0.871, 0.933}} \color{black} 0.308081 \\
 & 0.5 & {\cellcolor[rgb]{0.808, 0.898, 0.945}} \color{black} 0.238665 & {\cellcolor[rgb]{0.741, 0.867, 0.929}} \color{black} 0.320015 \\
 & 0.75 & {\cellcolor[rgb]{0.675, 0.831, 0.910}} \color{black} 0.401094 & {\cellcolor[rgb]{0.847, 0.922, 0.957}} \color{black} 0.187081 \\
 & 1.0 & {\cellcolor[rgb]{0.733, 0.863, 0.929}} \color{black} 0.327011 & {\cellcolor[rgb]{0.898, 0.949, 0.973}} \color{black} 0.123478 \\
\bottomrule
\end{tabular}

